MVFNet: Multipurpose Video Forensics Network using Multiple Forms of Forensic Evidence

While videos can be falsified in many different ways, most existing forensic networks are specialized to detect only a single manipulation type (e.g. deepfake, inpainting). This poses a significant issue as the manipulation used to falsify a video is not known a priori. To address this problem, we propose MVFNet - a multipurpose video forensics network capable of detecting multiple types of manipulations including inpainting, deepfakes, splicing, and editing. Our network does this by extracting and jointly analyzing a broad set of forensic feature modalities that capture both spatial and temporal anomalies in falsified videos. To reliably detect and localize fake content of all shapes and sizes, our network employs a novel Multi-Scale Hierarchical Transformer module to identify forensic inconsistencies across multiple spatial scales. Experimental results show that our network obtains state-of-the-art performance in general scenarios where multiple different manipulations are possible, and rivals specialized detectors in targeted scenarios.

==> figures/failure_modes.tex <==
\begin{figure*}[!t]
	\centering
	\setlength{\fboxsep}{0pt}
	\begin{minipage}[t]{1.0\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\parbox{0.150\textwidth}{\centering\smallerr Forged\\Video Frame}}
		\fbox{\parbox{0.150\textwidth}{\centering\smallerr Ground-truth Mask}}
		\fbox{\parbox{0.150\textwidth}{\centering\smallerr Our\\Predicted Mask}}
		\fbox{\parbox{0.300\textwidth}{\centering\smallerr Condition or\\Reasons of Failure}}
		\smallskip\smallskip
	\end{minipage}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_56_inappropriate.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_56_inappropriate_gt.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_56_inappropriate_pred.jpg}}}
		\makebox[0.300\textwidth][c]{\raisebox{16pt}{\smallerr New manipulation + Abnormal content}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_70_map_pixels_to_black.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_70_map_pixels_to_black_gt.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_70_map_pixels_to_black_pred.jpg}}}
		\makebox[0.300\textwidth][c]{\raisebox{16pt}{\smallerr New manipulation + Mapping pixels in region to black}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_92_altering_text.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_92_altering_text_gt.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_92_altering_text_pred.jpg}}}
		\makebox[0.300\textwidth][c]{\raisebox{16pt}{\smallerr New manipulation + Altering texts}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_126_very_subtle_text_modification.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_126_very_subtle_text_modification_gt.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_126_very_subtle_text_modification_pred.jpg}}}
		\makebox[0.300\textwidth][c]{\raisebox{16pt}{\smallerr New manipulation + Very subtle + Text modifications}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_138_too_small.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_138_too_small_gt.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_138_too_small_pred.jpg}}}
		\makebox[0.300\textwidth][c]{\raisebox{16pt}{\smallerr Too small}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_194_manip_region_too_smooth.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_194_manip_region_too_smooth_gt.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_194_manip_region_too_smooth_pred.jpg}}}
		\makebox[0.300\textwidth][c]{\raisebox{16pt}{\smallerr Manipulated region too smooth}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_216_combo_chains_of_editing_ops.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_216_combo_chains_of_editing_ops_gt.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_216_combo_chains_of_editing_ops_pred.jpg}}}
		\makebox[0.300\textwidth][c]{\raisebox{16pt}{\smallerr Unseen chains of editing operations}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_234_combo_chains_of_editing_ops.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_234_combo_chains_of_editing_ops_gt.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/failure_modes/videosham_234_combo_chains_of_editing_ops_pred.jpg}}}
		\makebox[0.300\textwidth][c]{\raisebox{16pt}{\smallerr Unseen chains of editing operations}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\caption{
		This figure shows cases where our network failed to identify forgeries. Further analysis is provided in Sec.~\ref{sec:failure_modes}.
	}
	\label{fig:failure_modes}
\end{figure*}



==> figures/ffe_arch.tex <==
\begin{figure*}[!h]
	\pullup
	\centering
	\includegraphics[width=1.0\linewidth]{figures/ffe_diagram}
	\caption{This figure shows the details of the Spatial Forensic Residual Feature Extractor.}
	\label{fig:ffe_arch}
	\pullupp
\end{figure*}

==> figures/front_page_graphic.tex <==

\begin{figure}[!h]
    \centering
    \setlength{\fboxsep}{0pt}
    \begin{minipage}[c]{0.53\linewidth}
        \centering
        \makebox[0.140\textwidth]{}
        \makebox[0.260\textwidth]{\small Authentic}
        \makebox[0.260\textwidth]{\small Forged}
        \makebox[0.260\textwidth]{\small Predicted Mask}
        \smallskip
    \end{minipage}

	\vspace*{-0.2\baselineskip}

    \begin{minipage}[ct]{0.53\linewidth}
        \centering
        \setlength{\fboxrule}{0pt}
		\makebox[0.140\textwidth][r]{\raisebox{9pt}{\small Deepfake\hspace{2pt}}}
        \fbox{\includegraphics[width=0.260\textwidth]{{figures/qualitative_results/frame_deepfake2}}}
        \fbox{\includegraphics[width=0.260\textwidth]{{figures/qualitative_results/gt_deepfake2}}}
        \fbox{\includegraphics[width=0.260\textwidth]{{figures/qualitative_results/vf2_deepfake2}}}
        \smallskip
    \end{minipage}

    \vspace*{-0.2\baselineskip}

    \begin{minipage}[c]{0.53\linewidth}
    	\centering
    	\setlength{\fboxrule}{0pt}
    	\makebox[0.140\textwidth][r]{\raisebox{9pt}{\small Inpainting\hspace{2pt}}}
    	\fbox{\includegraphics[width=0.260\textwidth]{{figures/qualitative_results/frame_inpainting2}}}
    	\fbox{\includegraphics[width=0.260\textwidth]{{figures/qualitative_results/gt_inpainting2}}}
    	\fbox{\includegraphics[width=0.260\textwidth]{{figures/qualitative_results/vf2_inpainting2}}}
    	\smallskip
    \end{minipage}

	\vspace*{-0.2\baselineskip}

    \begin{minipage}[c]{0.53\linewidth}
        \centering
        \setlength{\fboxrule}{0pt}
        \makebox[0.140\textwidth][r]{\raisebox{9pt}{\small Splicing\hspace{2pt}}}
        \fbox{\includegraphics[width=0.260\textwidth]{{figures/qualitative_results/frame_videosham}}}
        \fbox{\includegraphics[width=0.260\textwidth]{{figures/qualitative_results/gt_videosham}}}
        \fbox{\includegraphics[width=0.260\textwidth]{{figures/qualitative_results/vf2_videosham}}}
        \smallskip
    \end{minipage}

    \vspace*{-0.8\baselineskip}

	\caption{\label{fig:front_page_graphics} Sample video forgery localization results obtained using our proposed network on videos modified by deepfaking (Top), removing an object with inpainting (Middle), and splicing in an object (Bottom). \TODO{change this to a better graphic}}

	%In this figure, we show three example video frames. These are deepfake (top), adding an object (middle), and removing an object (bottom). Using our proposed network described in this paper, we are able to both detect these video frames to be manipulated and accurately localize the falsified region (predicted mask).}

	%\caption{\label{fig:front_page_graphics} In this figure, we show three video examples in which a human face is deepfaked (top), objects are added (middle), and objects are removed (bottom). Using our proposed network described in this paper, we are able to both detect that these video frames are manipulated and accurately localize the falsified region (predicted mask).}

    \vspace*{-\baselineskip}

\end{figure}

==> figures/front_page_graphic_v1.tex <==
\pullup\pullup\pullup\pullup\pullup
\begin{figure*}[!h]
	\centering
	\setlength{\fboxsep}{0pt}
	\begin{minipage}[t]{1.0\textwidth}
		\setlength{\fboxrule}{0pt}
		\makebox[0.140\textwidth]{}
		\makebox[0.100\textwidth]{\smallerr Input}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Spatial\\Evidence}}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Temporal\\Evidence}}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Spatio-Temporal\\Multi-Res.}}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Attention-Refined\\Feats.}}
		\makebox[0.100\textwidth]{\smallerr Output}
		\makebox[0.100\textwidth]{\smallerr GT}
		\smallskip
	\end{minipage}\hfill

	\vspace*{-0.1\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{0pt}
		\makebox[0.140\textwidth][r]{\raisebox{8pt}{\smallerr Editing\hspace{2pt}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_input_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_spat_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_temp_1}}}
		\fbox{\parbox[t]{0.100\textwidth}{\centering\includegraphics[width=0.056\textwidth]{{figures/intermediate_layers/videosham_spatio_temp_multi_res_1}}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_final_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_pred_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_gt_1}}}
		\smallskip
	\end{minipage}\hfill

	\vspace*{-0.1\baselineskip}

	\begin{comment}
	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{0pt}
		\makebox[0.140\textwidth][r]{\raisebox{8pt}{\smallerr Splice+Edit\hspace{2pt}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_input_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_spat_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_temp_2}}}
		\fbox{\parbox[t]{0.100\textwidth}{\centering\includegraphics[width=0.056\textwidth]{{figures/intermediate_layers/videosham_spatio_temp_multi_res_2}}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_final_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_pred_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/videosham_gt_2}}}
		\smallskip
	\end{minipage}

	\vspace*{-0.1\baselineskip}
	\end{comment}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\begin{comment}
	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{0pt}
		\makebox[0.140\textwidth][r]{\raisebox{8pt}{\smallerr Inpaint\hspace{2pt}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_input_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_spat_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_temp_1}}}
		\fbox{\parbox[t]{0.100\textwidth}{\centering\includegraphics[width=0.056\textwidth]{{figures/intermediate_layers/inpainting_spatio_temp_multi_res_1}}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_final_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_pred_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_gt_1}}}
		\smallskip
	\end{minipage}

	\vspace*{-0.1\baselineskip}
	\end{comment}

	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{0pt}
		\makebox[0.140\textwidth][r]{\raisebox{8pt}{\smallerr Inpaint\hspace{2pt}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_input_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_spat_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_temp_2}}}
		\fbox{\parbox[t]{0.100\textwidth}{\centering\includegraphics[width=0.056\textwidth]{{figures/intermediate_layers/inpainting_spatio_temp_multi_res_2}}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_final_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_pred_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/inpainting_gt_2}}}
		\smallskip
	\end{minipage}

	\vspace*{-0.1\baselineskip}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{0pt}
		\makebox[0.140\textwidth][r]{\raisebox{8pt}{\smallerr Deepfake\hspace{2pt}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_input_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_spat_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_temp_1}}}
		\fbox{\parbox[t]{0.100\textwidth}{\centering\includegraphics[width=0.056\textwidth]{{figures/intermediate_layers/deepfake_spatio_temp_multi_res_1}}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_final_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_pred_1}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_gt_1}}}
		\smallskip
	\end{minipage}

	\vspace*{-0.1\baselineskip}

	\begin{comment}
	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{0pt}
		\makebox[0.140\textwidth][r]{\raisebox{8pt}{\smallerr Deepfake\hspace{2pt}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_input_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_spat_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_temp_2}}}
		\fbox{\parbox[t]{0.100\textwidth}{\centering\includegraphics[width=0.056\textwidth]{{figures/intermediate_layers/deepfake_spatio_temp_multi_res_2}}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_final_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_pred_2}}}
		\fbox{\includegraphics[width=0.100\textwidth]{{figures/intermediate_layers/deepfake_gt_2}}}
		\smallskip
	\end{minipage}

	\end{comment}

	\label{fig:front_page_graphics}
	\caption{\TODO{Write this caption}}

	\pullupp\pullupp\pullupp\pullupp\pullupp\pullupp\pullupp\pullup
\end{figure*}

==> figures/front_page_graphic_v3.tex <==
\begin{table}
	\centering
	\resizebox{\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {|m{15mm}|m{19mm}|m{18mm}|m{18mm}|m{18mm}|m{18mm}|m{18mm}|m{18mm}|m{18mm}|},
				row{1} = {c},
				row{2} = {c},
				row{3} = {c},
				row{4} = {c},
				row{5} = {c},
				cell{1}{1} = {r=2}{},
				cell{1}{2} = {r=2}{},
				cell{1}{3} = {c=4}{c},
				cell{1}{7} = {c=2}{c},
				cell{1}{9} = {r=2}{},
				vline{2-4,8,10} = {1}{},
				vline{4-9} = {2}{},
				vline{2-10} = {3-5}{},
				hline{2} = {3-8}{},
				hline{3} = {-}{},
			}

			{Forgery\\Type} & {Forged\\Video Frame} & Forensic Modalities &  &  &  & Multi-Scale Analysis &  & {Ground Truth}\\
			&  & {Spatial\\Forensic} & {Spatial\\Context} & {Temporal\\Forensic} & {Temporal\\Opt. Flow} & {Coarse-Scale\\Feature} & {Fine-Scale\\Feature} & \\
			\raisebox{11pt}{Editing}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_3_input}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_3_spat_foren}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_3_spat_ctxt}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_3_temp_res}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_3_optflow_res}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_3_coarse}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_3_fine}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_3_gt}}}
			\\
			\raisebox{11pt}{Inpainting}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_2_input}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_2_spat_foren}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_2_spat_ctxt}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_2_temp_res}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_2_optflow_res}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_2_coarse}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_2_fine}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/inpaint_2_gt}}}
			\\
			\raisebox{11pt}{Deepfake}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/deepfake_2_input}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/deepfake_2_spat_foren}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/deepfake_2_spat_ctxt}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/deepfake_2_temp_res}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/deepfake_2_optflow_res}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/deepfake_2_coarse}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/deepfake_2_fine}}}
			& \mbox{\hspace{-3pt}\includegraphics[width=0.170\textwidth]{{figures/intermediate_layers/deepfake_2_gt}}}
		\end{tblr}
	}
	\
\end{table}

==> figures/intermediate_results.tex <==
\begin{figure*}[!t]
	\centering
	\setlength{\fboxsep}{0pt}
	\begin{minipage}[t]{1.0\textwidth}
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][s]{}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Forged\\Video Frame}}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Spatial Forensic\\Residuals}}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Spatial RGB Context}}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Temporal Forensic\\Residuals}}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Optical Flow\\Residuals}}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Coarse\\Features}}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Fine\\Features}}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Predicted Mask}}
		\fbox{\parbox{0.100\textwidth}{\centering\smallerr Grouth-\\Truth Mask}}
		\smallskip
	\end{minipage}

	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][r]{\raisebox{12pt}{\smallerr Vid.Sham}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_2_input}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_2_spat_foren}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_2_spat_ctxt}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_2_temp_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_2_optflow_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_2_coarse}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_2_fine}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_2_pred}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_2_gt}}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][r]{\raisebox{12pt}{\smallerr Vid.Sham}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_3_input}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_3_spat_foren}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_3_spat_ctxt}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_3_temp_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_3_optflow_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_3_coarse}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_3_fine}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_3_pred}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/videosham_3_gt}}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][r]{\raisebox{12pt}{\smallerr Inpaint}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_4_input}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_4_spat_foren}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_4_spat_ctxt}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_4_temp_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_4_optflow_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_4_coarse}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_4_fine}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_4_pred}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_4_gt}}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][r]{\raisebox{12pt}{\smallerr Inpaint}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_1_input}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_1_spat_foren}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_1_spat_ctxt}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_1_temp_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_1_optflow_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_1_coarse}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_1_fine}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_1_pred}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.05625\textwidth]{{figures/intermediate_layers/inpaint_1_gt}}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][r]{\raisebox{15pt}{\smallerr Deepfake}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_1_input}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_1_spat_foren}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_1_spat_ctxt}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_1_temp_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_1_optflow_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_1_coarse}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_1_fine}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_1_pred}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_1_gt}}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][r]{\raisebox{15pt}{\smallerr Deepfake}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_3_input}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_3_spat_foren}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_3_spat_ctxt}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_3_temp_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_3_optflow_res}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_3_coarse}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_3_fine}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_3_pred}}}
		\fbox{\includegraphics[width=0.100\textwidth, height=0.075\textwidth]{{figures/intermediate_layers/deepfake_3_gt}}}
	\end{minipage}
	\vspace*{-1.15\baselineskip}

	\caption{
		Intermediate layers' results are shown for different manipulation types, Splicing/Editing, Inpainting, and Deepfake. We see that for splicing/editing, the spatial features are more effective at uncovering forgery, while the temporal features are inadequate. For inpainting, temporal features are much more helpful in detecting anomalies than spatial features. And for deepfakes, both features are useful in detecting and localizing deepfakes. Further analysis is provided in Sec.~\ref{sec:intermediate_results}.
	}
	\label{fig:intermediate_results}

\end{figure*}



==> figures/results_on_authentic.tex <==
\begin{figure*}[!t]
	\centering
	\setlength{\fboxsep}{0pt}
	\begin{minipage}[t]{1.0\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][s]{}
		\fbox{\parbox{0.150\textwidth}{\centering\smallerr Forged\\Video Frame}}
		\fbox{\parbox{0.150\textwidth}{\centering\smallerr Our\\Predicted Mask}}
		\fbox{\parbox{0.150\textwidth}{\centering\smallerr Our\\Detection Score}}
		\fbox{\parbox{0.150\textwidth}{\centering\smallerr Authentic\\Video Frame}}
		\fbox{\parbox{0.150\textwidth}{\centering\smallerr Our\\Predicted Mask}}
		\fbox{\parbox{0.150\textwidth}{\centering\smallerr Our\\Detection Score}}
		\smallskip\smallskip
	\end{minipage}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr Davis Edit}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-editing_18_manip_1.000}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-editing_18_manip_1.000_pred}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 1.000}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-editing_19_real_0.049.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-editing_19_real_0.049_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.049}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr Davis Splice}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-splicing_12_manip_1.000.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-splicing_12_manip_1.000_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 1.000}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-splicing_13_real_0.375.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-splicing_13_real_0.375_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.375}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr Davis Splice}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-splicing_2_manip_0.996.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-splicing_2_manip_0.996_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.996}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-splicing_3_real_0.737.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/davis-splicing_3_real_0.737_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.737}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr VideoSham}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_116_manip_0.444.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_116_manip_0.444_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.444}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_117_real_0.005.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_117_real_0.005_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.005}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr VideoSham}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_2_manip_0.859.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_2_manip_0.859_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.859}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_3_real_0.305.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_3_real_0.305_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.305}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr VideoSham}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_30_manip_0.999.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_30_manip_0.999_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.999}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_31_real_0.006.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/videosham_31_real_0.006_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.006}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr Deepfake}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_14_manip_0.933.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_14_manip_0.933_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.933}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_15_real_0.024.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_15_real_0.024_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.024}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr Deepfake}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_50_manip_1.000.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_50_manip_1.000_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 1.000}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_51_real_0.057.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_51_real_0.057_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.057}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr Deepfake}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_6_manip_0.718.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_6_manip_0.718_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.718}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_7_real_0.003.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/ffpp-fsh_7_real_0.003_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.003}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr Inpainting}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_78_manip_0.971.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_78_manip_0.971_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.971}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_79_real_0.352.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_79_real_0.352_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.352}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr Inpainting}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_20_manip_0.283.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_20_manip_0.283_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.283}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_21_real_0.273.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_21_real_0.273_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.273}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-0.7pt}
		\makebox[0.070\textwidth][c]{\raisebox{16pt}{\smallerr Inpainting}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_86_manip_0.770.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_86_manip_0.770_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.770}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_87_real_0.05.jpg}}}
		\fbox{\includegraphics[width=0.150\textwidth, height=0.0844\textwidth]{{figures/authentic_loc_results/inpaint-e2fgvi_87_real_0.05_pred.jpg}}}
		\makebox[0.150\textwidth][c]{\raisebox{16pt}{\smallerr 0.050}}
	\end{minipage}
	\vspace*{-0.9\baselineskip}

	\caption{
		This figure shows our network's output on manipulated videos and their corresponding unmanipulated copies. As evident here and in the experiments presented in our main paper, our network can not only detect manipulated media, but also accurately classify authentic ones to be real. Further analysis is provided in Sec.~\ref{sec:results_on_authentic}.
	}
	\label{fig:results_on_authentic}
\end{figure*}



==> figures/supp_result_deepfake_dfd.tex <==
\newpage
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/more_loc_results/deepfake_DeepFakeDetection}

	\vspace*{-0.5\baselineskip}

	\caption{Localization results for deepfake detection are illustrated, highlighting the comparative effectiveness of various methods. Our \ournetworkname approach consistently provides precise localizations that closely match the Ground Truth. VideoFACT shows a small degree of accuracy. VIDNet achieves correct localization sporadically, with success in very few select cases. The remaining methods—DVIL, MVSS-Net, ManTra-Net, and FSG—largely fail to localize the specific regions of manipulation, often erroneously marking either the entire body or unrelated areas within the frame.}

	\label{fig:supp_loc_res_dfd}

	\vspace*{-0.5\baselineskip}

\end{figure*}
\newpage

==> figures/supp_result_deepfake_f2f.tex <==
\newpage
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/more_loc_results/deepfake_Face2Face}

%	\vspace*{-0.5\baselineskip}

	\caption{The figure displays localization results for Face2Face deepfake detection, highlighting the superior performance of our \ournetworkname method, which consistently provides accurate localizations that closely match the Ground Truth. VideoFACT rarely captures the manipulated regions correctly, often missing the mark. VIDNet and DVIL achieve limited success, with correct localization in a minority of cases. The rest of the methods, including MVSS-Net, ManTra-Net, and FSG, largely fail to identify the manipulated areas accurately, with localizations that either miss or misattribute the forgeries.}

	\label{fig:supp_loc_res_f2f}

%	\vspace*{-0.5\baselineskip}

\end{figure*}
\newpage

==> figures/supp_result_deepfake_fsh.tex <==
\newpage
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/more_loc_results/deepfake_FSH}

%	\vspace*{-0.5\baselineskip}

	\caption{Comparative localization results for FaceShifter deepfake detection are depicted. Our \ournetworkname method demonstrates precise localization, closely aligning with the Ground Truth, while VideoFACT shows some capability to localize manipulated areas but with less specificity. VIDNet, although occasionally accurate, largely fails to consistently delineate the manipulated regions. DVIL, MVSS-Net, and ManTra-Net generally misidentify the extent of the manipulations, often erroneously attributing them to other areas or the entire body. FSG's localizations are overly broad and imprecise, significantly deviating from the targeted manipulations indicated by the Ground Truth.}

	\label{fig:supp_loc_res_fsh}

%	\vspace*{-0.5\baselineskip}

\end{figure*}
\newpage

==> figures/supp_result_editing.tex <==
\newpage
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/more_loc_results/editing}

%	\vspace*{-0.5\baselineskip}

	\caption{This figure compares the localization results for editing detection on the VMMP dataset. Our \ournetworkname method achieves the most accurate localization, closely reflecting the Ground Truth. VideoFACT shows competent localization capabilities, slightly less precise than \ournetworkname. VIDNet and DVIL, while generally effective, do not match the accuracy of VideoFACT and show a decline in performance. MVSS-Net impresses with successful localizations in the majority of cases but falls short in others. The remaining methods, ManTra-Net and FSG, largely fail to accurately localize the manipulations, with a tendency to either miss or incorrectly identify the edited regions.}

	\label{fig:supp_loc_res_editing}

%	\vspace*{-0.5\baselineskip}

\end{figure*}
\newpage

==> figures/supp_result_inpainting.tex <==
\newpage
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/more_loc_results/inpainting}

%	\vspace*{-0.5\baselineskip}

	\caption{This figure presents localization results from various methods for an inpainting detection challenge. Our \ournetworkname method exhibits accurate and consistent localization closely mirroring the Ground Truth. VideoFACT achieves decent results, albeit with less precision than \ournetworkname. Both VIDNet and DVIL demonstrate good performance, delivering results that are on-par with our method in terms of accuracy. Conversely, MVSS-Net, ManTra-Net, and FSG struggle to identify the manipulated areas correctly, frequently misplacing the localization or entirely missing the inpainted regions.}

	\label{fig:supp_loc_res_inpainting}

%	\vspace*{-0.5\baselineskip}

\end{figure*}
\newpage

==> figures/supp_result_inpainting_e2fgvi.tex <==
\newpage
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/more_loc_results/vf_inpaint_E2FGVI}

	\vspace*{-0.5\baselineskip}

	\caption{This figure displays localization results for inpainting detection on the DAVIS-E2FGVI dataset. Our \ournetworkname approach outperforms others by producing localization masks that closely match the Ground Truth, with high precision and minimal false detections. VIDNet and DVIL demonstrate reasonable accuracy, effectively capturing the manipulated regions with some minor imprecisions. VideoFACT, while detecting the general area of manipulation, tends to generate overly broad masks, leading to a significant amount of false positives. The results from MVSS-Net, ManTra-Net, and FSG show a marked lack of accuracy, failing to provide useful localization in most cases and indicating a substantial departure from the Ground Truth.}

	\label{fig:supp_loc_res_e2fgvi}

	\vspace*{-0.5\baselineskip}

\end{figure*}
\newpage

==> figures/supp_result_inpainting_fuseformer.tex <==
\newpage
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/more_loc_results/vf_inpaint_FuseFormer}

%	\vspace*{-0.5\baselineskip}

	\caption{Localization results for inpainting detection on the DAVIS-FuseFormer dataset are compared across various methods. The \ournetworkname approach, our proposed method, consistently yields localization masks that are tightly aligned with the Ground Truth, demonstrating high fidelity and specificity. VideoFACT, while identifying the area of manipulation, tends to overextend the localization boundaries beyond the actual region. VIDNet shows a moderate level of accuracy, capturing significant portions of the manipulated areas but with less precision. DVIL, although somewhat effective, produces inconsistent results with varying degrees of overgeneralization. MVSS-Net, ManTra-Net, and FSG exhibit poor performance, with ManTra-Net and FSG generating particularly extensive and inaccurate localizations that deviate significantly from the Ground Truth.}

	\label{fig:supp_loc_res_fuseformer}

%	\vspace*{-0.5\baselineskip}

\end{figure*}
\newpage

==> figures/supp_result_splicing.tex <==
\newpage
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/more_loc_results/splicing}

%	\vspace*{-0.5\baselineskip}

	\caption{Localization accuracy for splicing detection is evaluated across different methods on the VMMP dataset. \ournetworkname showcases a high degree of precision, closely matching the Ground Truth. VideoFACT, while reasonably effective, does not attain the same level of accuracy as \ournetworkname. VIDNet and DVIL display less precision compared to VideoFACT, with their performance varying across different cases. MVSS-Net excels in a majority of scenarios but sometimes fails to detect the manipulation entirely. ManTra-Net and FSG generally provide inaccurate localizations, often identifying incorrect regions or missing the splicing altogether.}

	\label{fig:supp_loc_res_splicing}

%	\vspace*{-0.5\baselineskip}

\end{figure*}
\newpage

==> figures/supp_result_videosham.tex <==
\newpage
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/more_loc_results/videosham}

%	\vspace*{-0.5\baselineskip}

	\caption{Comparative localization results for video manipulation detection on the Adobe VideoSham dataset (Splice+Edit). The Ground Truth column displays the actual manipulated areas, followed by the detection results from our method (\ournetworkname) and other leading approaches: VideoFACT, VIDNet, DVIL, MVSS-Net, ManTra-Net, and FSG. Our method demonstrates superior localization precision, closely mirroring the Ground Truth, with clear, well-defined boundaries and minimal false positives. VideoFACT and VIDNet exhibit moderate localization accuracy but with less distinct boundaries. DVIL and MVSS-Net present overgeneralized localizations with significant false positives, while ManTra-Net and FSG show mostly inaccurate detections.}

	\label{fig:supp_loc_res_videosham}

%	\vspace*{-0.5\baselineskip}

\end{figure*}
\newpage

==> figures/temporal_arch.tex <==
\begin{wrapfigure}{r}{0.55\textwidth}
	\includegraphics[width=1.0\linewidth]{figures/temporal_module_diagram_v2}

	\vspace*{-0.5\baselineskip}

	\caption{This figure shows the components of the Temporal Forensic Feature Module.}

	\label{fig:temporal_arch}

	\vspace*{-0.5\baselineskip}

\end{wrapfigure}

==> sections/Abstract_v0.tex <==
% Abstract_v0

\begin{abstract}
While videos can be falsified in several different ways, existing forensic networks are specialized to detect only a single manipulation.  This poses a significant problem, since the manipulation used to falsify a video is not known a priori.  To address this problem, we propose a \ournetworkname - a new network capable of detecting multiple video manipulations including inpainting, deepfakes, splicing, and local editing.  Our network accomplishes this by extracting a rich set of spatio-temporal features from a video.  These features are then pooled across multiple resolutions to create a sequence of multi-scale forensic embeddings, which are analyzed for inconsistencies that are indicative of fake content.  Experimental results show that our network can successfully detect video forgeries when multiple different manipulations are possible.  Furthermore, our network can perform comparably to or better than state-of-the-art specialized forensic networks when evaluated only against their target manipulation.

\keywords{Video forensics \and Forgery detection \and Multi-scale \and Self-attenion}
\end{abstract}

==> sections/Experiments_v0.tex <==
% Experiments_v0

\section{Experiments}
\label{sec:experiments}


\subsection{Experimental Setup}
\label{subsec:experimental_setup}



\subheader{Training}
To train our network, first we pretrain the spatial forensic residual module using the Video-ACID dataset~\cite{Video-ACID} and freeze it for the next phase.
Next, we pretrain all remaining parts of the network using only spliced and edited videos in the \pooleddsabrv-IND subset.
Finally, we train the entire network on the whole \pooleddsabrv-IND subset.
During the two final stages, we start all loss parameters at 1.0 and decay $\gamma$ by 0.95 and $\alpha$ by 0.80, while increase $\beta$ by 1.18 every epoch.
More details are available in the supplementary material.

\subheader{Testing}
To get a complete picture of how well our approach and others detect fake content in video, we present two comprehensive sets of experiments, benchmarking performance in the multi-manipulation and single-manipulation settings. Note that, for specialist methods, the forgery type is not known a priori in the multi-manipulation scenario but is known in the single-manipulation scenario. In each configuration, we show results for both in-distribution (\pooleddsabrv-IND) and out-of-distribution (\pooleddsabrv-OOD) data.

\subheader{Metrics}
To evaluate all methods, we use frame-level detection mAP and pixel-level localization F1 scores. For methods that do not offer localization, only detection scores are reported. For non-detection methods, frame-level detection scores are derived from the highest per-pixel detection probability, a common approach in prior works~\cite{DVIL, VIDNet, MVSS-Net, TruFor, ManTra-Net, FSG} to ensure a fair comparison.

\subheader{Competing Methods}
We compare against 9 state-of-the-art methods. These systems can be divided into four major groups:
1) Splicing and Editing detector and localizer: MVSS-Net~\cite{MVSS-Net}, MantraNet~\cite{ManTra-Net}, Forensic Similarity Graph (FSG)~\cite{FSG},
2) Inpainting localizer: Video Inpainting Detection Network (VIDNet)~\cite{VIDNet}, Deep Video Inpainting Localization (DVIL)~\cite{DVIL},
3) Deepfake detector: Self-Blended Images (SBI)~\cite{SBI}, Multi-Attentional Deepfake Detection (MADD~\cite{MADD}, Cross-Efficient-ViT (CE.ViT)~\cite{CE.ViT}, and
4) General video forgery detector: VideoFACT~\cite{VideoFACT}.
For fair comparisons, we re-trained selectively top-performing methods of each major group, except Deepfake, using the exact same multi-manipulation training data as ours.
We cannot adapt deepfake detectors because their data pipeline requires a face detector to locate a face, which is impossible in the multi-manipulation setting. Nonetheless, these systems are all trained using the exact same deepfake data as ours.
Additionally, to show that a naive combination of forensic modalities is ineffective in this scenario, we present results for an ensemble of the retrained best methods.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Results on Multi-Manipulation Setting}
\label{subsec:mult_manips_eval}

Here, we benchmarked our approach and others in the multi-manipulation setting. Our testing data is split into three categories:
1) in-distribution data (\pooleddsabrv-IND) with content distribution and manipulation techniques similar to those in the training data,
2) out-of-distribution data (\pooleddsabrv-OOD) with unseen content distribution and different manipulation algorithms (of the same forgery types) than those seen in training, and
3) VideoSham which contains both new manipulation types and methods.
Tab.~\ref{table:results_on_joint_dataset} shows that our approach achieves the strongest detection and localization performance on all categories.

In particular, on \pooleddsabrv-IND, we achieve 0.95 AUC for detection and 0.77 F1 for localization, a significant improvement over all competing methods. The second best result belongs to a retrained version of MVSS-Net. While this version performs well on the in-distribution subset, its performance is substantially lower on the out-of-distribution subset (\pooleddsabrv-OOD). In contrast, our approach retains strong performance, while significantly outperforming all others, when tested against new and unseen manipulations in \pooleddsabrv-OOD. This trend also holds true for the VideoSham~\cite{VideoSham} dataset, whose forgeries are professionally made to be highly realistic using a diverse and unknown set of advanced techniques. Despite its extremely challenging manipulations, we perform considerably better than other competing methods and those reported in~\cite{VideoSham}.


\input{tables/pooled_results}


These results suggest that MVSS-Net, as well as other retrained methods, likely overfit to the manipulation algorithms shown during training and do not generalize to new and unseen manipulation algorithms even though the type of manipulation remains similar.
%On the other hand, our network is intentionally designed to extract general features that capture evidence of manipulations and not training-data specific discriminative features.
Importantly, across all datasets, we also considerably outperform an ensemble of best-retrained detectors.
This is due to multiple novel innovations in our network, including: 1) the inclusion of a new forensic modality to expose manipulations which leave behind temporal inconsistencies, 2) the carefully designed network architecture to combine and analyze evidence across all forensic modalities, and 3) the sophisticated use of a multi-scale hierarchical transformer to analyze all forensic evidence at and across multiple resolutions.


%Our proposed approach achieves the best performance on both in-distribution and out-of-distribution data. Regarding results for the \pooleddsabrv-IND subsets, we significantly outperform other specialized and general methods. When we retrained the best competing networks of each category (Splice/Edit, Inpainting, Deepfake, and General) on our training data, this gap is shorten slightly in the case of VideoFACT (R), and significantly in the case of MVSS-Net (R). However, when evaluating these retrained systems on unseen, out-of-distribution data, their performance dropped substantially while our approach still retain very strong results. This shows that training on multiple types of video forgery is needed but insufficient to detect a broad spectrum of manipulations. Additionally, since we outperform the ensemble of all retrained methods, this suggests that our approach of using multi-scale hierarchical analysis on a broad set of forensic modalities  is a major contributor to our performance difference.

%\subheader{Adobe VideoSham Dataset}
%On Adobe VideoSham, our proposed approach achieves the best performance, outperforming the second best method (MVSS-Net). Additionally, all approaches comparatively obtained worse results on this dataset because its forgeries are professionally made to be highly realistic using a diverse and unknown set of advanced techniques. Despite these challenging circumstances, we performed considerably better than other competing methods and those reported in~\cite{VideoSham}, including human evaluators.

\subsection{Results on Single-Manipulation Setting}
\label{subsec:indiv_manips_eval}

\input{tables/inpainting_results}

Here, we also put \ournetworkname, a general algorithm, against other specialized methods in their own intended manipulation scenario. The following experiments show that we outperform competing targeted detectors even when evaluating against manipulation that they were designed for.


\subheader{Inpainting Forgeries Evaluation}
From the results shown in Tab.~\ref{table:inpainting_results},
we outperformed competing inpainting detection systems in terms of detection across all testing sets. In terms of localization, we performed better than others on all datasets with the exception of DAVIS-E2FGVI-HQ, where DVIL~\cite{DVIL} is slightly better (0.27 vs 0.21 F1). Notably, in some cases, the retraining of competing methods has an inverse effect on the performance of these systems. This is because existing system do not have the components and sophisticated analysis networks to exploit the benefits of our multi-manipulation training data. Specifically, while these systems~\cite{VIDNet, DVIL} all use some form of temporal analysis, they often overlook spatial evidence, that, if exploited intentionally and in combination with evidence from other forensic modalities, can be effective at detecting inpainting forgeries.


\subheader{Splicing and Editing Forgeries Evaluation}
Tab.~\ref{table:splicing_editing_results} shows that our approach achieves the best detection mAP score on all testing sets. We also obtained the best localization F1 score on all datasets except for VCMS, where we are second place.
Notably, our performance remains consistently strong on both in-distribution and out-of-distribution datasets.
By contrast, the strongest competitor on the in-distribution datasets, a retrained MVSS-Net, performs significantly worse on the out-of-distribution datasets.
This suggests that MVSS-Net is likely prone to overfitting and has issues generalizing. \input{tables/splicing_editing_results}
Additionally, VideoFACT~\cite{VideoFACT} and its retrained version performs well on both in-distribution and out-of-distribution data.
This is likely due to the fact that, like our network, this system is designed for general video forensics. However, the fact that VideoFACT does not leverage temporal traces nor multi-scale analysis contributes largely to its performance gap comparing to ours.



\subheader{Deepfake Forgeries Evaluation}
Tab.~\ref{table:deepfakes_results} shows the evaluation of our approach and others on detecting and localizing deepfaked videos. In the set of in-distribution data, we achieve the best performance on DFD \& F2F, and competitive with other approaches on DF. \input{tables/deepfakes_results}
%
When tested against new and unseen generation methods (NT, FS, FSH), our approach achieves first place in NT, second place in FSH, and is comparable with state-of-the-art deepfake detectors like UCF~\cite{UCF}, SPSL~\cite{LiuCVPR2021}, SRM~\cite{LuoCVPR2021}, and SBI~\cite{SBI}. Notably, while we did not train on NT or FS like other competing detectors, our approach is still able to obtain good performance on these datasets. Additionally, our network is general and can work on all video without needing a face detector to first locate a human face. Even though face detectors are ubiquitous, they can still miss-detect, which adds as a source of error for existing deepfake detectors.





















==> sections/FFEPretrain_v0.tex <==

\subsection{FFE Pretraining}
\label{subsec:ffe_pretrain}

\begin{equation}
    \mathcal{L}_{\text{F}} = \sum_{k} \frac{-\lambda_k}{2^{2k}} \sum_{i,j} \sum_{c}
    \log\left(\frac{\exp(\theta^{k,c}_{i,j})\mathbbm{1}(c=c^*)}{\sum_{c} \exp(\theta^{k,c}_{i,j})} %\mathbbm{1}_{c=c^*}
    \right)
\end{equation}

%\cdot \mathbbm{1}_{c=C}



We introduce a novel pretraining procedure for the Forensic Feature Extractor (FFE) by building upon the established method in multimedia forensics for obtaining general forensic features through training on the Camera Model (CM) ID task\citethis. Our innovation lies in the means of producing forensic embeddings, and a new, accompanying objective function. The input frame initially passes through the FFE's trunk, which includes its constrained conv. layer and its series of FIR blocks. In prior works\citethis, this set of features is often condensed into a single embedding vector representing the entire frame for classification. However, in our work, we aggregated forensic features into embeddings for each analysis windows at multiple scales using a multi-resolution pooling module, as described in Sec.~\ref{subsec:multi_res_joint_embedding}. The resulting embeddings at each scale are then parallelly put through their own classification heads to produce 2D maps, in which each element specifies the input frame's CM class. The learning objective is to ensure that all elements in this map correspond to the same true CM class, promoting consistency across all spatial embeddings at different scales. The loss function for each scale is defined as:
\begin{equation}
    \mathcal{L}_{\text{ffe}}^{(k)} = -\frac{1}{2^k \times 2^k} \sum_{i,j} \sum_{c}
    \log(\frac{\exp(M^{k,c}_{i,j})}{\sum_{c} \exp(M^{k,c}_{i,j})} \cdot \mathbbm{1}_{c=C})
\end{equation}
where $M^{k,c}_{i,j}$ is the classification map at scale $k$ and CM $c$, and $\mathbbm{1}_{c=C}$ is the indicator function that is 1 when $c$ is the correct CM $C$ and 0 otherwise. The overall pretraining loss combines these scale-losses into a weighted sum:
\begin{equation}
    \mathcal{L}_{\text{ffe}} = \sum_{k=1}^{K} w_{k} \mathcal{L}_{\text{ffe}}^{(k)}
\end{equation}
Post-training, we retain solely the trunk of the FFE and merge it into our larger network. This innovative pretraining method enhances the FFE’s capability for spatial inconsistency detection, significantly improving our ability to detect and localize spatial anomalies.

%% Reason why aggregating into single embedding is insufficient:
% 1. Loss of Spatial Information: Aggregating into a single embedding for the entire frame may lead to a loss of crucial spatial information. Forensic features can vary significantly across different regions of a frame, and a single embedding might not capture these local variations effectively. Our approach of using multi-scale analysis windows retains this local spatial information, providing a more detailed and accurate representation.

% 2. Limited Sensitivity to Small-Scale Manipulations: A single embedding representing the entire frame might not be sensitive enough to detect small-scale or subtle manipulations. By using multi-resolution pooling, our method can potentially detect finer details and inconsistencies that would be missed with a single, frame-wide embedding.

% 3. Difficulty in Localization: With a single embedding, localization of the manipulated region within a frame can be challenging. Multi-scale embeddings provide a more granular view, making it easier to pinpoint the exact location of inconsistencies, which is crucial for effective manipulation localization.

% 4. Over-Simplification of Complex Forensic Features: Video frames often contain complex forensic features that a single embedding may oversimplify. By employing a multi-resolution approach, our method can capture a richer and more nuanced set of features, leading to more accurate detection and analysis.

==> sections/Intro_v0.tex <==
% Intro_v1
%
\section{Introduction}
\label{sec:intro}



The ease with which videos can be convincingly modified or falsified poses an important misinformation threat to society. Powerful AI techniques enable the creation of visually convincing fake media.
%For example, deepfakes enable a user to replace the true face of a speaker in a video with a falsified face of a target speaker~\citethis.  Similarly, AI-based inpainting techniques enable the removal of any object from a video~\citethis.
In particular, deepfakes allows bad actors to assume and manipulate any facial identity~\cite{DeepFaceLab, Deepfakes, NeuralTextures, MegaFS}, and inpaiting enables the removal of any unwanted objects in a video~\cite{JointOpt, VINet, DFCNet, OPN}.

In addition to %these more recent
AI-based methods, traditional
%signal-processing-based
%video
manipulations, such as
%those commonly found in video editing software,
splicing and editing,
can still be effective at creating plausible fake videos. For example, inauthentic content can be added through splicing and green screening, or,
%Similarly, fake content can be further
modified by
%through operations such as
blurring, sharpening, resizing, rotation, etc.

To combat this, a variety of forensic authentication techniques have been developed.  Deepfakes in particular have received significant attention, resulting in the development of a broad set of approaches for detecting deepfake video~\cite{FF++, MesoNet, UCF, NiCVPR2022, CaoCVPR2022, LiuCVPR2021, LuoCVPR2021}.
More recently, several networks have been proposed to identify inpainted video regions~\cite{DVIL, VIDNet, YuICCV2021}.
% While video inpainting has received less attention, recent work has been proposed to identify inpainted video regions~\citethis.
Furthermore, though mostly examined within the context of images, a number of techniques have been proposed to detect content splicing and editing~\cite{ManTra-Net, Noiseprint, EXIFnet, MVSS-Net, FSG}.

\input{figures/front_page_graphic}
Despite this important body of forensic research,
there exists a crucial gap that has posed challenges in deploying video forgery detection systems in real-world scenarios. That is:
%the wide variety of possible video manipulations poses an important problem:
when examining a video in-the-wild, we do not know which manipulation may have been applied a priori.
%By contrast, existing video forensic detectors are designed to identify only a single specific type of manipulation.
%As a result, these detectors are not well suited to use in more general forensic scenarios.
%As a result, these detectors can produce inaccurate results in more general forensic scenarios.
As a result, it is difficult to get reliable results from any set of current specialized detectors.
For instance, a deepfake detector, designed to identify falsified faces, will fail to detect manipulations  such as
%splicing in a new backing scene
green-screening
or object removal using inpainting.

%For example, if inpainting was used to remove an object from the background of a person speaking, or if the the background was replaced by splicing, a deepfake detector will fail to identify that the video has been falsified since it is designed to identify falsified faces.
%
%For instance, when examining a video of a human speaker, a deepfake detector designed to identify falsified faces will fail to detect
%
% may fail to detect manipulations involving background changes such as splicing in a new backing scene or removing an object through inpainting.

%Because of this, there is a significant need for forensic networks that can detect multiple different manipulations.

%Nonetheless,
Creating a general solution to video forgery is highly non-trivial
%Detecting multiple different potential video manipulations is challenging
because not all manipulations leave behind the same form of evidence.  Some manipulations can be detected by examining spatially inconsistent intra-frame forensic traces~\cite{Tolosana2020IF, Nabi2022MS}.  By contrast, others introduce temporal inconsistencies that are identified by examining traces across frames~\cite{Shelke2021MTA, Nabi2022MS}.  As a result, it is necessary for a general approach to extract and analyze a broad set of both spatial and temporal features in order to detect a broad variety of manipulations.
%
%Furthermore, the size and shape of the manipulated content is not known a priori.  Hence, it is also important to analyze forensic evidence across multiple scales to accurately localize both large, small, and irregularly shaped fake regions.

\begin{comment}
%In this paper,
To this end,
we propose a new forensic network capable of detecting multiple different types of video forgery.
% 1.
Our network first gather a broad array of spatial and temporal features, including: forensic residual, RGB context, optical flow anomaly, and temporal residual features.
% 2.
Then, this rich set of spatio-temporal features are aggregated into forensic embeddings, each corresponds to different analysis windows at multiple scales using a novel Multi-Resolution Pooling approach.
% 3.
To accurately uncover subtle inconsistencies in these embeddings, we used a Transformer-based module to jointly analyze the full sequence of forensic embeddings and identify anomalous traces indicative of forgery.
% 4.
We trained our network on a challenging dataset, comprising of multiple manipulation types and diverse distributions of scene content.
% 5.
During extensive evaluation, our network not only excels in multi-manipulation scenarios but also demonstrates competitive performance in detecting specific forgeries, in both in-domain and cross-domain benchmarking datasets, rivaling specialized state-of-the-art systems.
%a rich set of spatio-temporal features, then uses them to create a sequence of forensic embeddings across multiple scales.
%Fake content is detected by analyzing these multi-scale spatio-temporal embeddings for evidence of localized forensic inconsistencies.
%
%This is facilitated %aided
%by a transformer-based self attention module that is able to jointly analyze the full sequence of forensic  embeddings, then identify those that correspond to anomalous or inconsistent traces that are indicative of forgery.
%Experimental results presented in this paper show that our network is able to detect multiple different video manipulations without requiring prior knowledge of which individual manipulation may have been used.
%%
%Furthermore, our network performs comparably to or better  than state-of-the-art specialized forensic networks when used to detect only a single possible manipulation such as inpainting, deepfakes, splicing, and editing.
\end{comment}


To address this, we propose \ournetworkname - a new forensic network capable of detecting multiple different video manipulations.  Our network gathers a rich set of spatio-temporal features, then uses them to create a sequence of forensic embeddings across multiple scales.
Fake content is detected by analyzing these multi-scale spatio-temporal embeddings for evidence of localized forensic inconsistencies.
%
This is facilitated %aided
by a transformer %-based self attention
module that is able to jointly analyze the full sequence of forensic  embeddings, then identify those that correspond to anomalous or inconsistent traces that are indicative of forgery.
Experimental results presented in this paper show that our network is able to detect multiple different video manipulations without requiring prior knowledge of which individual manipulation may have been used.
%
Furthermore, our network performs comparably to or better  than state-of-the-art specialized forensic networks when used to detect only a single possible manipulation such as inpainting, deepfakes, splicing, and editing.
%
%
%\vspace{0.25\baselineskip}
%\noindent
The novel contributions of our paper are: %as follows:
\begin{itemize}
	\item We propose a new forensic network able to detect and localize fake content in videos made by multiple different types of manipulation.

%	\item We improve the potency of our forensic feature extractor using a novel pretraining procedure and loss function.

%	\item We carefully design novel network components to specifically capture
%	a comprehensive set of spatio-temporal forensic features in order to detect multiple potential manipulations
	%
%	, including: forensic residual, RGB context, optical flow anomaly, and temporal residual features.
	% These include intra-frame features to capture spatial inconsistencies such as learned forensic residual features and RGB context features, as well as inter-frame features to capture temporal inconsistencies such as optical flow features and cross-frame residual difference features.


	\item Our network extracts and analyzes a comprehensive set of spatio-temporal forensic features in order to detect multiple potential manipulations,
%
including inter-frame forensic residual features, RGB context features, optical flow anomaly features, and intra-frame residual  features.

	\item From this rich set of features, we produce novel
	multi-scale joint forensic embeddings that enable us to detect and localize falsified content of all sizes and shapes.

	\item We then leverage the self-attention mechanism in our transformer module to contextualize all embeddings with one another and identify inconsistent ones that point to evidence of forgeries.

	\item We conduct a comprehensive set of experiments that demonstrate our network's superior ability to detect fake content in multi-manipulation scenarios, and rival or exceed  specialized state-of-the-art systems
	in single manipulation scenarios.
%	 can not only detect multiple video manipulations in general forensic scenarios, but it can also perform comparably to or better than existing specialized manipulation detectors when evaluated only on their target manipulation.


%\item We present a comprehensive set of experiments that show that our proposed network can not only detect multiple video manipulations in general forensic scenarios, but it can also perform comparably to or better than existing specialized manipulation detectors when evaluated only on their target manipulation.


\end{itemize}



%Furthermore, when our network is used to detect a only a single possible  manipulation, it performs comparably to or better than state-of-the-art specialized forensic networks designed to detect inpainting, deepfakes, splicing, and editing.




%Furthermore, our network is able to perform comparably to or better than state-of-the-art specialized forensic networks designed to detect inpainting, deepfakes, splicing, and editing.


% Furthermore, when used to detect a single manipulation, our network is able to perform comparably or better than state-of-the-art specialized forensic networks designed to detect inpainting, deepfakes, splicing, and editing.





\begin{comment}
Fake and manipulated videos pose an important misinformation threat.

There are a wide variety of different ways that a video can be falsified.

AI techniques such as deepfakes enable a user to replace the face of a speaker with that of another target speaker.  In response a number approaches have been proposed to detect deepfake videos.

Similarly, an object can be removed from a video using AI-based inpainting techniques.  While this problem has received less attention than the detection of deepfakes, recent work has been proposed to identify inpainted video regions.

In addition to these more recent AI-based manipulations, traditional signal-processing-based video editing operations, such as those commonly found in video editing software, can still be effectively used to create visually convincing videos.  For example, inauthentic content can be added through splicing and green screening.  Similarly, fake content can be further modified through operations such as blurring, sharpening, resizing, rotation, etc.
Though mostly examined within the context of image editing, a number of techniques have been proposed to detect content splicing and editing.




The wide variety of video manipulations, however, poses an important problem: we do not know what manipulations may have been applied to a video a priori.  By contrast, existing video forensic detectors are designed to identify only a single specific type of manipulation.  As a result, these detectors are not well suited to use in more general forensic scenarios.
For example, if inpainting was used to remove an object from the background of a person speaking, or if the the background was replaced by splicing, a deepfake detector will fail to identify that the video has been falsified since it is designed to identify falsified faces.

There is a significant need for forensic networks that can detect multiple different manipulations.  This is challenging, however, because not all manipulations leave behind the same forms of evidence.
Some manipulations can be detected by examining spatially inconsistent intra-frame forensic traces.  By contrast, others introduce temporally inconsistencies that are identified by examining enter-frame traces.
As a result, it is necessary for a forensic network to extract and analyze a broad set of both spatial and temporal features in order to detect a broader variety of different manipulations.

Furthermore, the size and shape of the manipulated content is not known a priori.  As a result, it is necessary to analyze forensic features across multiple scales ot accurately localize both large, small, and irregularly shaped fake regions.

In this paper, we propose a new forensic network capable of detecting multiple different video manipulations.  Our network gathers a rich set of spatiotemporal features, then uses them to create a sequence of forensic embeddings across multiple scales.
Fake content is detected by analyzing these multi-scale spatiotemporal embeddings for evidence of localized forensic inconsistencies.

This is aided by a transformer-based self attention module that is able to jointly analyze the full sequence of embeddings, then identify those that correspond to anomalous or inconstent features indicative of forgery.

As a result our network is able to detect multiple different video manipulations without requiring prior knowledge of which individual manipulation may have been used.  Furthermore, when used to detect a single manipulation, our network is able to perform comparably or better than state-of-the-art specialized forensic networks designed to detect inpainting, deepfakes, splicing, and editing.

\end{comment}

==> sections/Intro_v1.tex <==
\section{Introduction}
\label{sec:intro}

The ease with which videos can be convincingly modified or falsified poses an important misinformation threat to society. Powerful AI techniques enable the creation of visually convincing fake media.
%
In particular, deepfakes allows bad actors to assume and manipulate any facial identity~\cite{DeepFaceLab, Deepfakes, NeuralTextures, MegaFS}, and inpaiting enables the removal of any unwanted objects in a video~\cite{JointOpt, VINet, DFCNet, OPN}.
%
In addition to AI-based methods, traditional manipulations, such as splicing and editing, can still be effective at creating plausible fake videos. For example, inauthentic content can be added through splicing and green screening, or, modified by blurring, sharpening, resizing, rotation, etc.

To combat this, many specialized forensic authentication techniques have been developed. Notably, Deepfakes have received significant attention, resulting in the development of a broad set of approaches for detecting deepfaked video~\cite{FF++, MesoNet, UCF, NiCVPR2022, CaoCVPR2022, LiuCVPR2021, LuoCVPR2021}.
Additionally, several recent networks have been proposed to identify inpainted video regions~\cite{DVIL, VIDNet, YuICCV2021}.
%
Last but not least, though mostly examined within the context of images, a number of techniques have been proposed to detect content splicing and editing~\cite{ManTra-Net, Noiseprint, EXIFnet, MVSS-Net, FSG}.



These dedicated systems work by exploiting prior knowledge about their targeted manipulation. In particular, deepfake detectors assume the presence of a face and look for generative artifacts, specific to human facial anatomy \citethis; and inpainting localizers assume the absence of an object and look for inconsistencies in motion as a result of imperfect generation or occlusions. Because of this, the set of features that these systems are capable of learning do not span the ``space'' of those they are not designed to detect. Hence, existing video authentication systems are ill-equipped to detect a wide variety of manipulation types (e.g. deepfakes, inpainting, splicing, editing, etc.).


In order to address this crucial problem, it is necessary to not only leverage existing general forms of spatial forensic modalities,
%
but also develop new ones for traces that manifest themselves temporally.
%
Specifically, in this paper, we leverage spatially distributed forensic residual and RGB context as our foundational modalities, which are adept at identifying inconsistencies within the spatial domain of a video frame. These existing modalities have proven effective in detecting manipulations that alter the continuity of forensic microstructures inside a frame\citethis.
%
Complementing these, we introduce temporally distributed temporal residual and optical flow residual as novel forensic modalities. They focus on capturing anomalies in the temporal domain, such as irregular motion patterns or pixel value fluctuations that may not be visible in static frames. Unlike prior works\citethis, which attempted to model the anomalous and authentic sequences of temporal features directly, our novel approach circumvents the impracticality of learning all possible variations of abnormal and normal embedding sequences.
%

Since each forensic modality manifests a different type of evidence, the combination of them enables us to authenticate videos without any prior knowledge about the applied manipulation or the video itself. Additionally, by analyzing all modalities simultaneously, our system does not overlook any potential evidence that was previously under-explored by existing specialized approaches.

To this end, we propose \ournetworkname - the first network to integrate the use of multiple new and existing forensic modalities for accurately detecting and localizing a wide variety of video manipulation types (deepfake, inpainting, splicing and editing). For each forensic modality, we carefully designed individual feature extractor and performed pre-training (if necessary) to ensure maximum generalizability. In particular, we pretrained the spatial forensic residual module using a novel loss function that resulted in substantial gain in overall performance. Then, we designed a novel multi-scale hierarchical transformer module to intelligently combine and analyze all available evidence at different granularities and level of information so as to uncover inconsistent or anomalous regions of all shapes and sizes. Through a series of extensive experiments, we show that our network obtained state-of-the-art performance in multi-manipulation setting, in which the manipulation is not known a prior. And similarly, we out-performed specialist detectors on their targeted manipulation type in most benchmarks. To summarize, the novel contributions of our paper are:
\begin{itemize}
	\item We propose new forensic modalities - temporally distributed forensic residual and optical flow residual - to better extract temporal evidences. These new types of traces allow our network to detect a broad spectrum of forgeries containing temporal anomalies.
	\item We propose a new loss function to significantly boost the effectiveness of our spatial forensic residual module during its pretraining stage.
	\item We introduce \ournetworkname, the first network to incorporate multiple forensic modalities for detecting and localizing many forms of video forgery.
	\item We design a novel multi-scale hierarchical transformer module to combine and jointly analyze all forensic evidences at multiple scales and levels of information for indication of forgery.
	\item We conduct a comprehensive set of experiments that demonstrate our network's superior ability to detect fake content in multi-manipulation scenarios, and rival or exceed specialized state-of-the-art systems
	in single manipulation scenarios.
\end{itemize}







==> sections/Intro_v2.tex <==
\section{Introduction}
\label{sec:intro}

The ease with which videos can be convincingly modified or falsified poses an important misinformation threat to society. Powerful AI techniques enable the creation of visually convincing fake media.
%
In particular, deepfakes allows bad actors to assume and manipulate any facial identity~\cite{DeepFaceLab, Deepfakes, NeuralTextures, MegaFS}, and inpaiting enables the removal of any unwanted objects in a video~\cite{JointOpt, VINet, DFCNet, OPN}.
%
%In addition to AI-based methods,
Additionally,
traditional manipulations, such as splicing and editing, can still be effective at creating plausible fake videos. For example, inauthentic content can be added through splicing and green screening, or, modified by blurring, sharpening, resizing, rotation, etc.

\begin{comment}
To combat this, many specialized forensic authentication techniques have been developed. Notably, Deepfakes have received significant attention, resulting in the development of a broad set of approaches for detecting deepfaked video~\cite{FF++, MesoNet, UCF, NiCVPR2022, CaoCVPR2022, LiuCVPR2021, LuoCVPR2021}.
Additionally, several recent networks have been proposed to identify inpainted video regions~\cite{DVIL, VIDNet, YuICCV2021}.
%
Last but not least, though mostly examined within the context of images, a number of techniques have been proposed to detect content splicing and editing~\cite{ManTra-Net, Noiseprint, EXIFnet, MVSS-Net, FSG}.
\end{comment}


To combat this, many specialized forensic authentication techniques have been developed.  Deepfakes in particular have received significant attention, resulting in the development of a broad set of approaches for detecting deepfake video~\cite{FF++, MesoNet, UCF, NiCVPR2022, CaoCVPR2022, LiuCVPR2021, LuoCVPR2021}.
More recently, several networks have been proposed to identify inpainted video regions~\cite{DVIL, VIDNet, YuICCV2021}.
% While video inpainting has received less attention, recent work has been proposed to identify inpainted video regions~\citethis.
Furthermore, though mostly examined within the context of images, a number of techniques have been proposed to detect content splicing and editing~\cite{ManTra-Net, Noiseprint, EXIFnet, MVSS-Net, FSG}.

------

While these specialized systems work well on their targeted manipulation, they are not designed to generalize to other types of forgery.  This is because they implicitly or explicitly leverage information about their target manipulation to aid detection.  Furthermore, they extract forensic features designed specifically to expose evidence of their target manipulation as opposed to features that will work well in more general settings.
%For example, deepfake detectors assume the presence of a face and search for evidence of imperfect face generation \citethis.  Inpainting localizers assume that an object has been removed and search for motion inconsistencies caused by imperfect content generation \citethis.
%
%Furthermore, they only leverage modalities of forensic traces immediately usesful to detecting their target manipulation.


As a result, there is a crucial challenge exists when creating video forensic systems capable of operating in realistic scenarios: How should we detect forgeries when we don't know a prior what specific manipulation may have been used? 
%Furthermore, we often don't 
This problem necessitates the development general video forensic techniques able to detect multiple differe





As a result, there exists a crucial gap that has posed challenges in deploying video forgery detection systems in real-world scenarios. 


As a result, there exists a crucial gap that has posed challenges in deploying video forgery detection systems in real-world scenarios. That is:
%the wide variety of possible video manipulations poses an important problem:
when examining a video in-the-wild, we do not know which manipulation may have been applied a priori.
%By contrast, existing video forensic detectors are designed to identify only a single specific type of manipulation.
%As a result, these detectors are not well suited to use in more general forensic scenarios.
%As a result, these detectors can produce inaccurate results in more general forensic scenarios.
As a result, it is difficult to get reliable results from any set of current specialized detectors.
For instance, a deepfake detector, designed to identify falsified faces, will fail to detect manipulations  such as
%splicing in a new backing scene
green-screening
or object removal using inpainting.


The focus on specialized detectors has led researchers to overlook certain forensic feature modalities that can prove useful both general and specialized settings.

In this paper, we propose MVFAST



-

As a result, it is necessary to capture a broad set of forensic feature modalities that collectively are able to capture evidence of a broad variety of manipulations.  Importantly, features extraced from a particular modality should be general enough that they can be used to detect multiple manipulations that leave evidence in that modality

Network should make minimal to no prior assumptions about scene content, manpulation type, shape or size of fake region

In this paper, we propose MVFAST
which is able to detect multiple different video manipulations without prior knowledge of which (if any) were applied
To do this, we extract information from multiple spatially and temporally distributed forensic feature modalities.  Key among these is temporal forensic residuals, which is a new forensic modality that, to the best of our knowledge, has not been utilized by prior work.
Because not all manipulations leave behind common forms of evidence, our network jointly analyzes evidence from all of these modalities to expose a wide range of forgeries
Furthermore,
somethign about multi-scale transformer
Experimental results show

Novelties
(0) New network able detect multiple different manipulations at once
(1) Capture multiple forensic modalites in one network using features genearal enough.
(2) introduce new modality of forensic features
(3) Multi-scale transformer
(4) Experiments (and mention new dataset). also mention in and out of distribution






-----



These dedicated systems work by exploiting prior knowledge about their targeted manipulation. In particular, deepfake detectors assume the presence of a face and look for generative artifacts, specific to human facial anatomy \citethis; and inpainting localizers assume the absence of an object and look for inconsistencies in motion as a result of imperfect generation or occlusions. Because of this, the set of features that these systems are capable of learning do not span the ``space'' of those they are not designed to detect. Hence, existing video authentication systems are ill-equipped to detect a wide variety of manipulation types (e.g. deepfakes, inpainting, splicing, editing, etc.).


In order to address this crucial problem, it is necessary to not only leverage existing general forms of spatial forensic modalities,
%
but also develop new ones for traces that manifest themselves temporally.
%
Specifically, in this paper, we leverage spatially distributed forensic residual and RGB context as our foundational modalities, which are adept at identifying inconsistencies within the spatial domain of a video frame. These existing modalities have proven effective in detecting manipulations that alter the continuity of forensic microstructures inside a frame\citethis.
%
Complementing these, we introduce temporally distributed temporal residual and optical flow residual as novel forensic modalities. They focus on capturing anomalies in the temporal domain, such as irregular motion patterns or pixel value fluctuations that may not be visible in static frames. Unlike prior works\citethis, which attempted to model the anomalous and authentic sequences of temporal features directly, our novel approach circumvents the impracticality of learning all possible variations of abnormal and normal embedding sequences.
%

Since each forensic modality manifests a different type of evidence, the combination of them enables us to authenticate videos without any prior knowledge about the applied manipulation or the video itself. Additionally, by analyzing all modalities simultaneously, our system does not overlook any potential evidence that was previously under-explored by existing specialized approaches.

To this end, we propose \ournetworkname - the first network to integrate the use of multiple new and existing forensic modalities for accurately detecting and localizing a wide variety of video manipulation types (deepfake, inpainting, splicing and editing). For each forensic modality, we carefully designed individual feature extractor and performed pre-training (if necessary) to ensure maximum generalizability. In particular, we pretrained the spatial forensic residual module using a novel loss function that resulted in substantial gain in overall performance. Then, we designed a novel multi-scale hierarchical transformer module to intelligently combine and analyze all available evidence at different granularities and level of information so as to uncover inconsistent or anomalous regions of all shapes and sizes. Through a series of extensive experiments, we show that our network obtained state-of-the-art performance in multi-manipulation setting, in which the manipulation is not known a prior. And similarly, we out-performed specialist detectors on their targeted manipulation type in most benchmarks. To summarize, the novel contributions of our paper are:
\begin{itemize}
	\item We propose new forensic modalities - temporally distributed forensic residual and optical flow residual - to better extract temporal evidences. These new types of traces allow our network to detect a broad spectrum of forgeries containing temporal anomalies.
	\item We propose a new loss function to significantly boost the effectiveness of our spatial forensic residual module during its pretraining stage.
	\item We introduce \ournetworkname, the first network to incorporate multiple forensic modalities for detecting and localizing many forms of video forgery.
	\item We design a novel multi-scale hierarchical transformer module to combine and jointly analyze all forensic evidences at multiple scales and levels of information for indication of forgery.
	\item We conduct a comprehensive set of experiments that demonstrate our network's superior ability to detect fake content in multi-manipulation scenarios, and rival or exceed specialized state-of-the-art systems
	in single manipulation scenarios.
\end{itemize}







==> sections/Intro_v3.tex <==
\section{Introduction}
\label{sec:intro}

The ease with which videos can be convincingly modified or falsified poses an important misinformation threat to society. Powerful AI techniques enable the creation of visually convincing fake media.
%
In particular, deepfakes allows bad actors to assume and manipulate any facial identity~\cite{DeepFaceLab, Deepfakes, NeuralTextures, MegaFS}, and inpaiting enables the removal of any unwanted objects in a video~\cite{JointOpt, VINet, DFCNet, OPN}.
%
%In addition to AI-based methods,
Additionally,
traditional manipulations, such as splicing and editing, can still be effective at creating plausible fake videos. For example, inauthentic content can be added through splicing and green screening, or, modified by blurring, sharpening, resizing, rotation, etc.

\begin{comment}
	To combat this, many specialized forensic authentication techniques have been developed. Notably, Deepfakes have received significant attention, resulting in the development of a broad set of approaches for detecting deepfaked video~\cite{FF++, MesoNet, UCF, NiCVPR2022, CaoCVPR2022, LiuCVPR2021, LuoCVPR2021}.
	Additionally, several recent networks have been proposed to identify inpainted video regions~\cite{DVIL, VIDNet, YuICCV2021}.
	%
	Last but not least, though mostly examined within the context of images, a number of techniques have been proposed to detect content splicing and editing~\cite{ManTra-Net, Noiseprint, EXIFnet, MVSS-Net, FSG}.
\end{comment}


To combat this, many specialized forensic authentication techniques have been developed.  Deepfakes in particular have received significant attention, resulting in the development of a broad set of approaches for detecting deepfake video~\cite{FF++, MesoNet, UCF, NiCVPR2022, CaoCVPR2022, LiuCVPR2021, LuoCVPR2021}.
More recently, several networks have been proposed to identify inpainted video regions~\cite{DVIL, VIDNet, YuICCV2021}.
% While video inpainting has received less attention, recent work has been proposed to identify inpainted video regions~\citethis.
Furthermore, though mostly examined within the context of images, a number of techniques have been proposed to detect content splicing and editing~\cite{ManTra-Net, Noiseprint, EXIFnet, MVSS-Net, FSG}.


While these specialized systems work well on their targeted manipulation, they are not designed to generalize to other types of forgery.  This is because they implicitly or explicitly leverage information about their target manipulation to aid detection.  Furthermore, they extract forensic features designed specifically to expose evidence of their target manipulation as opposed to features that will work well in more general settings.
%For example, deepfake detectors assume the presence of a face and search for evidence of imperfect face generation \citethis.  Inpainting localizers assume that an object has been removed and search for motion inconsistencies caused by imperfect content generation \citethis.
%
%Furthermore, they only leverage modalities of forensic traces immediately usesful to detecting their target manipulation.


As a result, it is difficult to get reliable results from any set of current specialized detectors when examining videos in-the-wild because we do not know which manipulation may have been applied a priori.
For instance, a deepfake detector, designed to identify falsified faces, will fail to detect manipulations  such as green-screening or object removal using inpainting.

\begin{comment}
As a result, there exists a crucial gap that has posed challenges in deploying video forgery detection systems in real-world scenarios. That is:
%the wide variety of possible video manipulations poses an important problem:
when examining a video in-the-wild, we do not know which manipulation may have been applied a priori.
%By contrast, existing video forensic detectors are designed to identify only a single specific type of manipulation.
%As a result, these detectors are not well suited to use in more general forensic scenarios.
%As a result, these detectors can produce inaccurate results in more general forensic scenarios.
As a result, it is difficult to get reliable results from any set of current specialized detectors.
For instance, a deepfake detector, designed to identify falsified faces, will fail to detect manipulations  such as
%splicing in a new backing scene
green-screening
or object removal using inpainting.

The focus on specialized detectors has led researchers to overlook certain forensic feature modalities that can prove useful both general and specialized settings.
\end{comment}

Therefore, to address this problem, it is necessary to exploit a collective broad set of forensic feature types, or, modalities,
that collectively are able to capture evidence of a broad variety of manipulations.
%
Importantly, features extraced from a particular modality should be general enough that they can be used to detect multiple types of forgery that leave evidence in that modality.
%
Additionally, to detect manipulated videos in the wild, no prior assumptions are to be made about scene content, manpulation type, shape or size of fake region.

In this paper, we propose \ournetworkname, a network capable of
detecting multiple different video manipulations without any prior knowledge about the applied method.
To do this, we extract information from multiple spatially and temporally distributed forensic feature modalities.
%
Key among these is temporal forensic residuals, which is a new forensic modality that, to the best of our knowledge, has not been utilized by prior work.
%
Because not all manipulations leave behind common types of evidence, our network jointly analyzes all feature evidence from every modalities to expose a wide range of forgery types.
%
Furthermore, to detect manipulations of all shapes and sizes, we performed our joint analysis using a novel multi-scale hierarchical transformer module. This module uses multiple transformers, which are connected together in a hierarchical manner, at different scales to identify inconsistencies of forensic features across scales.
%
Through a series of extensive experiments, we show that our network obtained state-of-the-art performance in multi-manipulation setting, in which the manipulation is not known a priori.
And similarly, we out-performed specialist detectors on their targeted manipulation type in most benchmarks. To summarize, the novel contributions of our paper are:
\begin{enumerate}
	\item We propose a new network to detect and localize multiple types of manipulation without any prior knowledge about the applied method.
	\item To accomplish this, we jointly analyze over all evidence from a broad set of forensic modalities.
	\item We introduce the temporal forensic residuals, a new forensic modality, to better capture anomalous temporal changes in forensic microstructures.
	\item multi-scale hierarchical transformer
	\item Experiments (and mention new dataset). also mention in and out of distribution
\end{enumerate}






\begin{comment}
-----



These dedicated systems work by exploiting prior knowledge about their targeted manipulation. In particular, deepfake detectors assume the presence of a face and look for generative artifacts, specific to human facial anatomy \citethis; and inpainting localizers assume the absence of an object and look for inconsistencies in motion as a result of imperfect generation or occlusions. Because of this, the set of features that these systems are capable of learning do not span the ``space'' of those they are not designed to detect. Hence, existing video authentication systems are ill-equipped to detect a wide variety of manipulation types (e.g. deepfakes, inpainting, splicing, editing, etc.).


In order to address this crucial problem, it is necessary to not only leverage existing general forms of spatial forensic modalities,
%
but also develop new ones for traces that manifest themselves temporally.
%
Specifically, in this paper, we leverage spatially distributed forensic residual and RGB context as our foundational modalities, which are adept at identifying inconsistencies within the spatial domain of a video frame. These existing modalities have proven effective in detecting manipulations that alter the continuity of forensic microstructures inside a frame\citethis.
%
Complementing these, we introduce temporally distributed temporal residual and optical flow residual as novel forensic modalities. They focus on capturing anomalies in the temporal domain, such as irregular motion patterns or pixel value fluctuations that may not be visible in static frames. Unlike prior works\citethis, which attempted to model the anomalous and authentic sequences of temporal features directly, our novel approach circumvents the impracticality of learning all possible variations of abnormal and normal embedding sequences.
%

Since each forensic modality manifests a different type of evidence, the combination of them enables us to authenticate videos without any prior knowledge about the applied manipulation or the video itself. Additionally, by analyzing all modalities simultaneously, our system does not overlook any potential evidence that was previously under-explored by existing specialized approaches.

To this end, we propose \ournetworkname - the first network to integrate the use of multiple new and existing forensic modalities for accurately detecting and localizing a wide variety of video manipulation types (deepfake, inpainting, splicing and editing). For each forensic modality, we carefully designed individual feature extractor and performed pre-training (if necessary) to ensure maximum generalizability. In particular, we pretrained the spatial forensic residual module using a novel loss function that resulted in substantial gain in overall performance. Then, we designed a novel multi-scale hierarchical transformer module to intelligently combine and analyze all available evidence at different granularities and level of information so as to uncover inconsistent or anomalous regions of all shapes and sizes. Through a series of extensive experiments, we show that our network obtained state-of-the-art performance in multi-manipulation setting, in which the manipulation is not known a prior. And similarly, we out-performed specialist detectors on their targeted manipulation type in most benchmarks. To summarize, the novel contributions of our paper are:
\begin{itemize}
	\item We propose new forensic modalities - temporally distributed forensic residual and optical flow residual - to better extract temporal evidences. These new types of traces allow our network to detect a broad spectrum of forgeries containing temporal anomalies.
	\item We propose a new loss function to significantly boost the effectiveness of our spatial forensic residual module during its pretraining stage.
	\item We introduce \ournetworkname, the first network to incorporate multiple forensic modalities for detecting and localizing many forms of video forgery.
	\item We design a novel multi-scale hierarchical transformer module to combine and jointly analyze all forensic evidences at multiple scales and levels of information for indication of forgery.
	\item We conduct a comprehensive set of experiments that demonstrate our network's superior ability to detect fake content in multi-manipulation scenarios, and rival or exceed specialized state-of-the-art systems
	in single manipulation scenarios.
\end{itemize}
\end{comment}






==> sections/MultiResEmbed_v0.tex <==
% MultiResEmbed_v1_MCS
%
%\subsection{Multi-Resolution Joint Embedding Module}
\subsection{Multi-Scale Spatio-Temporal Embeddings}
\label{subsec:multi_res_joint_embedding}

% Overview
% What is the problem we are trying to solve, what is the intuition, what is the solution
% Goal/Motivation: Since we are looking for "inconsistencies", we need to look at the correlation of an analysis region with the rest of the frame.
% Problem: The volume of residual spatial and temporal anomaly features is very dense and can be very large (H x W x C). Additionally, the spatio-temporal feature at a particular location (i, j) has small and limited receptive field, which often leads to higher degree of variability in feature space when compared to other near-by locations.
% Solution: Adaptively pool at multiple resolutions to create analysis windows with large receptive field where the statistics of the spatio-temporal features inside is stable and more useful when looking for anomalies.
% Effect: Allow for reasoning (done by the Transformer) over analysis windows of multiple scales, and for the ability to be agnostic to variable video resolutions through training. (edited)



%In prior works \citethis, a challenge usually appears when aggregating forensic traces over analysis windows. Larger window provides better estimate of the forensic microstructures, but this comes at cost of missing small or irregularly shaped falsified regions. This is exacerbated in our case where the shape and size of both the input video and the fake region is not known a priori. Therefore, to be able to detect and localize fake content of arbitrary shape and size, we need to analyze the video at multiple spatial resolutions. 

%To this goal, we first join the Spatial Residual Features, $S_{t}$ and the Temporal Residual Features, $T_{t}$, then adaptively pool at multiple resolutions to aggregate the residual features over large-to-small analysis windows:
%

%\hrulefill

Fake regions are typically identified by comparing forensic features aggregated over an analysis window and identifying inconsistencies.  This presents an inherent challenge: larger windows provide more estimates of forensic traces, but at the cost of missing small or irregularly sized forgery regions.  To overcome this, we pool forensic features across multiple resolutions, then create a set of multi-scale spatio-temporal feature embeddings 
as shown in Fig~\ref{fig:multi_res_pooling_arch}.

We form %a sequence of 
spatio-temporal feature embeddings $\psi_t^{(k)}$ at scale $k$ by concatenating the spatial and temporal forensic features, then pooling using the adaptive pooling operation $\Gamma$~\cite{AdaptiveMaxPool2d} such that
%
\begin{equation}
    \begin{split}
        \psi_t^{(k)}(i,j)= \Gamma(S_{t} \concat T_{t} \;,\; \omega^{(k)}(i,j))
    \end{split}
\end{equation} 
%
%where $\Gamma$ is the adaptive pooling operation \citethis, 
where $\omega^{(k)}(i,j)$ is the pooling kernel at location $(i,j)$ at scale $k$. 
%
%Here, the size of each linear dimension of $\omega^{(k)}$ is equal to $2^k$ times the linear dimension of $\omega^{(1)}$, the baseline 
Each linear dimension of $\omega^{(k)}$ is equal to $2^k$ times the corresponding dimension of the baseline kernel $\omega^{(1)}$.
%
%The resulting features at each scale $k$ are then concatenated to form the a sequence of multi-resolution spatio-temporal feature embeddings $\xi$ such that
%
Corresponding embeddings across each scale $k$ are then concatenated to form the a sequence of multi-scale spatio-temporal feature embeddings $\xi$ such that
%
%Multi-Resolution Joint Features $\xi_{t}$:
%
\begin{equation}
    \begin{split}
        \xi_{t}(i,j) = \; & \psi_t^{(1)}(p^{(1)},q^{(1)}) \; \concat \; \psi_t^{(2)}(p^{(2)},q^{(2)}) \; \concat \ldots   \\
                       & \ldots  \; \concat \; \psi_t^{(K)}(p^{(K)},q^{(K)}), 
%		\xi_{t}(i,j) = \; & \psi_t^{(0)}(i,j) \; \concat \; \psi_t^{(1)}(i,j) \; \concat \ldots   \\
%                       & \ldots  \; \concat \; \psi_t^{(k)}(i,j) 
    \end{split}
\end{equation}
% \begin{equation}
%     \begin{split}
%         \xi_{t}(i,j) = \bigoplus_{k=0}^{K} \psi_t^{(k)}(p^{k},q^{k})
%     \end{split}
% \end{equation}
%
where $p^{(k)}= \lfloor \tfrac{i-1}{2^k} \rfloor + 1$ and $q^{(k)}= \lfloor \tfrac{j-1}{2^k} \rfloor + 1$.
In practice, we pool across $K=3$ different scales.
%In practice, we use 3 different scales $k \in \{3, 4, 5\}$, resulting in 3 sets of features with size 8x8, 16x16, and 32x32 respectively.






==> sections/MultiScaleHierTransformer_v0.tex <==
\subsection{Multi-Scale Hierarchical Transformer Module} %(new improved version)
\label{subsec:multi_scale_hier_transformer_mod}

\input{figures/multi_res_pooling}

In order to identify a broad spectrum of fake content in video, it is necessary to look for inconsistencies across all forensic modalities. However, since the sizes and shapes of the faked regions are not known a priori,
%
oversized analysis windows risk overlooking smaller forgeries or inaccurately localizing irregularly shaped ones. Conversely, overly small windows could misinterpret natural minor variations in forensic traces as manipulations.
%
%if we choose the size of our analysis windows too big, we may miss smaller forgeries or poorly localize irregularly shaped ones, and if it's too small, we may mistake regions with naturally minor variation in forensic traces as being manipulated.
%
Additionally, we cannot totally disregard information from smaller analysis windows because they hold the key for delineating forgeries' sophisticated boundaries.


To address this,
we introduce an innovative approach employing Multi-Scale Hierarchical Transformers.
Initially, evidence from all modalities is combined into a comprehensive dense set of joint forensic features,
$\xi_t$, such that:
\begin{equation}
	\xi_{t} = F_t \concat C_t \concat T_t \concat O_t
\end{equation}
%
Then, our module employs adaptive pooling, $\Gamma$, to distill this feature set into embeddings at various spatial scales $\psi_t^{(k)}(i,j)$, and analyze them in a coarse-to-fine manner:
\begin{equation}
	\psi_t^{(k)}(i,j)= \Gamma(\xi_t \;,\; \omega^{(k)}(i,j)), \;\; k \in S=\lbrace 1, 2, \cdots, L \rbrace
\end{equation}
where $\omega^{(k)}(i,j)$ is the pooling kernel at location $(i,j)$ at scale $k$.
%
In order to facilitate analysis within and across scales, the transformer at each scale needs three sets of input: current and prior scale's pooled embeddings, and previous scale's insights from the previous transformer. However, since these inputs have different resolutions, they must first pass through the Resolution-Aware Connector, which ensures coherent feature integration across scales:
\begin{equation}
	B_t^{(k)} = \psi_t^{(k)} + \left[ \omega(G_t^{(k-1)}, 2) + \omega(\psi_t^{(k-1)}, 2) \right]
\end{equation}
in which $B_t^{(k)}$ is the output Resolution-Aware Connector and $\omega(X, Y)$ is the bilinear interpolation applying on input $X$ with scaling factor $Y$. Finally, $B_t^{(k)}$ is given to a series of transformer encoder blocks to form the output embeddings at the current scale:
\begin{equation}
	G_t^{(k)} = Z_t^{(k, \ell)} \circ Z_t^{(k, \ell - 1)} \circ \cdots \circ Z_t^{(k, 1)}(B_t^{(k)} + E^{(k)})
\end{equation}
where $Z_t^{(k, \ell)}$ is the $\ell^{\text{th}}$ encoder block of scale $k$ and $E^{(k)}$ is the vector of learned positional embeddings for scale $k$.

Hence, at each scale, the transformer blocks utilize the self-attention mechanism to look for embeddings exhibiting inconsistent features in context of all other embeddings.
%
Furthermore, due to skip-connections, higher blocks in the hierarchy have access to insights from lower ones.
%
This strategy enables our network to utilize finer-scale information for precise localization while minimizing false positives through insights from broader scales.

We note that while some other forensic networks use multi-scale analysis, their approaches are substantially different from ours. Some works\citethis either naively combine features from multiple scales, or fail to exploit cross-scale insights\citethis. Others\citethis enable some degree of information flow across scales, but do not utilize self-attention to contextualize inconsistencies within or among them. While a smaller portion of works\citethis use some forms of attention mechanism, they are designed to weight the relative importance of forensic features, not identifying regions with anomalies in context of other regions. Most notably, the prevalent approach in multi-scale forensic analysis operate in a fine-to-coarse manner\citethis. As our ablation experiments show, this is highly suboptimal as it predisposes the network to false alarms at the finest scale, which can then propagate through out the system. By adopting a coarse-to-fine approach, our network can isolate local false alarms using more reliable indications of forgery and localize complex fake regions boundaries with greater precision.































==> sections/MultiScaleHierTransformer_v1.tex <==
\subsection{Multi-Scale Hierarchical Transformer Module} %(new improved version)
\label{subsec:multi_scale_hier_transformer_mod}



%After collecting all modalities of forensic features, we must jointly analyze them to identify fake content. 

After collecting evidence from all forensic feature modalities, we concatentate them form joint forensic features $\xi_t$ such that 
\begin{equation}
	\xi_{t} = F_t \concat C_t \concat T_t \concat O_t
\end{equation}
and use them to identify fake content. 
%

%
Fake regions are typically identified by comparing forensic features aggregated over an analysis window and identifying inconsistencies.  This presents an inherent challenge: larger windows provide more accurate estimates of forensic traces
 and improved false alarm suppression
, but at the cost of missing small or irregularly sized forgery regions.  

%This presents an inherent challenge since we don't know the size and shape of fake content a priori.  If analysis windows are too small, minor local variations will cause false alarms.  However if analysis windows are too big, we will miss small fake regions and achieve poor localization accuracy.  


To overcome this, we propose a novel multi-scale hierarchical transformer module to analyze joint feature embeddings. This module first pools these joint features into embeddings at multiple spatial scales, then analyzes them in a coarse to fine manner.  The transformer encoders at a particular scale use their self-attention mechanism to look for meaningful embedding disparities in the context of one another. However, they also share information across multiple scales to leverage the more accurate localization ability of finer scales and the false alarm suppression ability of larger scales.


Module combines all four forensic feature modalities, pools them into embeddings at multiple spatial scales, then analyzes them in a coarse to fine manner


---
[START HERE]

Module combines all four forensic feature modalities and pools them into embeddings at multiple spatial scales.  The embedding $\psi_t^{(k)}$ at scale $k$ is formed by using the adaptive pooling operation $\Gamma$~\cite{AdaptiveMaxPool2d} such that
%
\begin{equation}
    \begin{split}
        \psi_t^{(k)}(i,j)= (F_t \concat C_t \concat T_t \concat O_t \;,\; \omega^{(k)}(i,j))
    \end{split}
\end{equation} 
where $\omega^{(k)}(i,j)$ is the pooling kernel at location $(i,j)$ at scale $k$. 
Each linear dimension of $\omega^{(k)}$ is equal to $2^k$ times the corresponding dimension of the baseline kernel $\omega^{(1)}$.

%  ^{(k)}

There is a transformer at each scale.

Let $A^{(k)}$ denote the output of the transformer encoder block at scale $k$.

Input to transformer at scale $k$ is $B^{(k)}$

$B^{(k)}$ is created by combining the output of the transformer at the previous scale $A^{(k-1)}$ withe the pooled embeddings at the current scale $\psi_t^{(k)}$ and previous scale $\psi_t^{(k-1)}$.  

Because these do not have the same dimensionality, we join them using a component we call a resolution aware connector.  This adds transformer output and embeddings at the previous scale, then doubles their spatial size through bilinear interpolation so that they can be added to the embeddings at the current scale such that
\begin{equation}
        B_t^{(k)}= \rho(\psi_t^{(k)} + A_t^{(k)}) \convolve \kappa + \psi_t^{(k+1)}
\end{equation} 
where $\rho(\cdot)$ is the zero interleaving operation and $\kappa$ is the bilinear interpolation kernel.


 bilearly interpolates them to the 

they must be joined using a resolution aware connector 










[END HERE]

----

Our module begins by pooling the $\psi_t^{(k)}$ at scale $k$ by concatenating the spatial and temporal forensic features, then pooling using the adaptive pooling operation $\Gamma$~\cite{AdaptiveMaxPool2d} such that
%
\begin{equation}
    \begin{split}
        \psi_t^{(k)}(i,j)= \Gamma(S_{t} \concat T_{t} \;,\; \omega^{(k)}(i,j))
    \end{split}
\end{equation} 
%
%where $\Gamma$ is the adaptive pooling operation \citethis, 
where $\omega^{(k)}(i,j)$ is the pooling kernel at location $(i,j)$ at scale $k$. 
%
%Here, the size of each linear dimension of $\omega^{(k)}$ is equal to $2^k$ times the linear dimension of $\omega^{(1)}$, the baseline 
Each linear dimension of $\omega^{(k)}$ is equal to $2^k$ times the corresponding dimension of the baseline kernel $\omega^{(1)}$.



\input{figures/multi_res_pooling}

%%%%%%%%%%%%%%%%%%
\hrulefill
%%%%%%%%%%%%%%%%%%


In order to identify a broad spectrum of fake content in video, it is necessary to look for inconsistencies across all forensic modalities. However, since the sizes and shapes of the faked regions are not known a priori,
%
oversized analysis windows risk overlooking smaller forgeries or inaccurately localizing irregularly shaped ones. Conversely, overly small windows could misinterpret natural minor variations in forensic traces as manipulations.
%
%if we choose the size of our analysis windows too big, we may miss smaller forgeries or poorly localize irregularly shaped ones, and if it's too small, we may mistake regions with naturally minor variation in forensic traces as being manipulated.
%
Additionally, we cannot totally disregard information from smaller analysis windows because they hold the key for delineating forgeries' sophisticated boundaries.


To address this,
we introduce an innovative approach employing Multi-Scale Hierarchical Transformers.
Initially, evidence from all modalities is combined into a comprehensive dense set of joint forensic features,
$\xi_t$, such that:
\begin{equation}
	\xi_{t} = F_t \concat C_t \concat T_t \concat O_t
\end{equation}
%
Then, our module employs adaptive pooling, $\Gamma$, to distill this feature set into embeddings at various spatial scales $\psi_t^{(k)}(i,j)$, and analyze them in a coarse-to-fine manner:
\begin{equation}
	\psi_t^{(k)}(i,j)= \Gamma(\xi_t \;,\; \omega^{(k)}(i,j)), \;\; k \in S=\lbrace 1, 2, \cdots, L \rbrace
\end{equation}
where $\omega^{(k)}(i,j)$ is the pooling kernel at location $(i,j)$ at scale $k$.
%
In order to facilitate analysis within and across scales, the transformer at each scale needs three sets of input: current and prior scale's pooled embeddings, and previous scale's insights from the previous transformer. However, since these inputs have different resolutions, they must first pass through the Resolution-Aware Connector, which ensures coherent feature integration across scales:
\begin{equation}
	B_t^{(k)} = \psi_t^{(k)} + \left[ \omega(G_t^{(k-1)}, 2) + \omega(\psi_t^{(k-1)}, 2) \right]
\end{equation}
in which $B_t^{(k)}$ is the output Resolution-Aware Connector and $\omega(X, Y)$ is the bilinear interpolation applying on input $X$ with scaling factor $Y$. Finally, $B_t^{(k)}$ is given to a series of transformer encoder blocks to form the output embeddings at the current scale:
\begin{equation}
	G_t^{(k)} = Z_t^{(k, \ell)} \circ Z_t^{(k, \ell - 1)} \circ \cdots \circ Z_t^{(k, 1)}(B_t^{(k)} + E^{(k)})
\end{equation}
where $Z_t^{(k, \ell)}$ is the $\ell^{\text{th}}$ encoder block of scale $k$ and $E^{(k)}$ is the vector of learned positional embeddings for scale $k$.

Hence, at each scale, the transformer blocks utilize the self-attention mechanism to look for embeddings exhibiting inconsistent features in context of all other embeddings.
%
Furthermore, due to skip-connections, higher blocks in the hierarchy have access to insights from lower ones.
%
This strategy enables our network to utilize finer-scale information for precise localization while minimizing false positives through insights from broader scales.

We note that while some other forensic networks use multi-scale analysis, their approaches are substantially different from ours. Some works\citethis either naively combine features from multiple scales, or fail to exploit cross-scale insights\citethis. Others\citethis enable some degree of information flow across scales, but do not utilize self-attention to contextualize inconsistencies within or among them. While a smaller portion of works\citethis use some forms of attention mechanism, they are designed to weight the relative importance of forensic features, not identifying regions with anomalies in context of other regions. Most notably, the prevalent approach in multi-scale forensic analysis operate in a fine-to-coarse manner\citethis. As our ablation experiments show, this is highly suboptimal as it predisposes the network to false alarms at the finest scale, which can then propagate through out the system. By adopting a coarse-to-fine approach, our network can isolate local false alarms using more reliable indications of forgery and localize complex fake regions boundaries with greater precision.































==> sections/PropApproach_v0.tex <==
% PropApproach_v0

\section{Proposed Approach}
\label{sec:propApproach}



%In order to detect multiple different manipulations, we design our network's architecture to explicitly model a diverse set of  forensic features.

An overview of our network's architecture is shown in Fig.~\ref{fig:overview_arch}.
%
In order to detect a variety of video manipulations, it is critical to search for multiple forms of evidence that a video has been falsified.  To accomplish this, our network is explicitly designed to detect a diverse set of intra-frame spatially distributed features and inter-frame temporal features.  This is done using two parallel spatial and temporal forensic modules at the beginning of our network.

All features are then combined and pooled across multiple resolutions to produce a sequence of multi-scale spatio-temporal embeddings. This enables our network to detect fake regions with varied sizes and irregular shapes.  The sequence embeddings are analyzed by a transformer module, whose self-attention mechanism enables our network to expose inconsistent embeddings indicative of fake video regions.  The transformer output is passed to separate detection and localization modules that produce detection scores and localization masks respectively.


\begin{comment}



Our network's architecture  is explicitly designed to enable it to  detect a variety of different video manipulations.  To accomplish this,



% Network overview
Figure \citethis illustrates the architecture of our proposed network, designed for the detection and localization of diverse types of video content manipulations. The architecture is tailored to operate independently of specific prior knowledge about the manipulation techniques employed.

Central to our approach are specialized modules tasked with identifying intra-frame spatial and inter-frame temporal inconsistencies. These modules generate comprehensive feature sets, which are subsequently fused in a multi-resolution joint embeddings module. This fusion is critical for enhancing the network's capability to detect and localize forgeries across a range of scales and complexities.

Following this, the sequence of multi-scale spatio-temporal embeddings is subjected to a deep Transformer-based self-attention module. This module leverages the self-attention mechanism to effectively discern relationships between embeddings, crucial for accurate localization of manipulated regions. The output from the self-attention module is then fed into a fully connected layer, producing the final frame-level detection scores and pixel-level localization masks.

Subsequent sections will detail the specific motivations and functionalities of each individual module within our network architecture.
%





\begin{comment}
Placeholder text

\subsection{Spatial Module}


The spatial module of our network produces two separate sets of intermediate features: forensic residual features and RGB context features.  These are produced by two parallel branches within the spatial forensic module

The first branch produces forensic residual features.  These are higher level forensic features learned from low-level prediction residuals.  Different forms of residual features have been widely used throughout forensics because they capture statistical relationships between pixels within a local neighborhood


Low-level prediction residuals remove the visual content from an image, while


--

\subhead{Forensic Residual Features}
The first branch produces forensic residual features that capture information about a video frame's source and processing history.  At a high level, the use of forensic features learned from prediction residuals is a popular and widely successful strategy used in forensics.  Prediction residuals suppress an image or video frame's content while preserving noise-like microstructures that are induced by the process that formed it (e.g. digital camera, AI generator) and by manipulations subsequently used to edit it (add examples).

%This type of features has been widely used throughout forensics to capture statistical relationships with


Rather than using a fixed linear high-pass filter, our network produces a set of learned residuals using a constrained convolutional layer proposed by Bayar and Stamm \cite{ }.
%
%This layer contains $L$ learnable prediction filters $\phi$.  Each filter is used to predict pixel values, then these predictions are subtracted from the true values to produce a residual according to
%\begin{equation}
%\res^{(i)}=\vframe * (\delta - \phi^{(i)})
%\end{equation}
%where $*$ denotes convolution and $\delta$ is a unit impulse, i.e. the convolutional identity element.  The resulting $L$ different sets of residuals contain
%
This layer contains $L$ learnable prediction filters $\phi$, whose output is subtracted from the central pixel value within each filter window.  This produces a set of residuals $\res^{(i)}$ corresponding to the $i^{th}$ filter such that\begin{equation}
\res^{(i)}=\vframe * (\delta - \phi^{(i)})
\end{equation}
where $*$ denotes convolution and $\delta$ is a unit impulse, i.e. the convolutional identity element.
The resulting $L$ different sets of residuals capture a diverse set of microstructure information that a single filter has difficulty capturing.  Furthermore, since these filters are learned, they adapt specifically to capture low-level forensic information that can best be exploited by higher network layers.

Next, higher-level forensic features are learned from these low-level residuals.  This is done by passing the residuals through a network consisting of \textbf{[FILL IN NETWORK ARCHITECTURE HERE]}.



%To obtain forensic residual features, our network first passes a video frame $vframe$ through a constrained convolutional layer.  This layer produces $L$ distinct residual fields by using

%First, a video frame $\vframe$ is passed through a constrained convolutional layer consisting of $L$ distinct learnable prediction residual filters.  This results in a set of $L$ low-level learned forensic residual fields $\res$, such that
%\begin{equation}
%\res^{(i)}=\vframe * (\delta + \phi^{(i)})
%\end{equation}

% These low-level learned residuals are then passed to


\subhead{RGB Context Features}

The second branch


While forensic residual features are the primary means of identifying inconsistencies in the source and processing history of different parts of a frame, local information about the RGB content of a scene can provide important context to the network when making decisions based on these residual features.  For example, it is well known that the distribution of forensic residual features can change based on a number of factors, including local texture information, the presence of edges, compression strength, etc.~\cite{placeholder}.




While forensic residual features are the primary means of extracting spatially distributed forensic information from a video frame, RGB information is still important.  It is well known that the distribution of forensic residual features can change based on a number of factors, including local texture information, the presence of edges, compression, etc.  Similarly, the quality of forensic information varies throughout a scene based on local content~\cite{placeholder}.  For example,

content of the scene~\cite{placeholder}.  Similarly

the texture information, p

 content within a local region~\cite{placeholder}.  Similarly, cont


\subsection{Temporal Module}

\subsection{Multi-Scale Joint Forensic Embeddings}



\begin{equation}
\psi_t^{(k)}(i,j)= \Gamma(\res_t \oplus \contxt_t, \omega^{(k)}(i,j))
\end{equation}



%\begin{equation}
%\xi(i,j)= \embedscalepos{0} \; \oplus \; \embedscalepos{1} \; \oplus \;  \embedscalepos{2}
%\end{equation}



\begin{align}
\xi(i,j)= \; & \embedscalepos{0} \; \oplus \; \embedscalepos{1} \; \oplus \ldots   \\
& \ldots  \; \oplus \; \embedscalepos{k}
\end{align}

where $p^{(k)}= \lfloor \tfrac{i-1}{2^k} \rfloor + 1$ and $q^{(k)}= \lfloor \tfrac{j-1}{2^k} \rfloor + 1$

\subsection{Temporal Unit}

\end{comment}

==> sections/PropApproach_v1.tex <==
\section{Proposed Approach}
\label{sec:propApproach}

In order to detect a variety of different video manipulations, it is critical to search for multiple forms of evidence that a video has been falsified.
Our network does this by using parallel branches to extract four different forensic feature modalities: spatial forensic residuals, spatial RGB context features, temporal forensic residuals, and optical flow residuals.
We note that temporal forensic residuals are a novel feature modality that we introduce for the first time in this work.
Additionally, while optical flow has been directly used in prior forensic networks, ours is the first to instead use optical flow residuals.
%
Next, we combine evidence from all forensic modalities and search for locally anomalous evidence that indicate a manipulated region.
%
We do this using a novel multi-scale hierarchical transformer module, which uses self-attention to analyze all evidence simultaneously across different scale
to accurately identify anomalous or inconsistent content regardless of their shapes and sizes.
%
These high-level insights are then passed to two subnetworks, one produces a detection score (how likely is the video frame faked), and the other produces a localization mask (where the fake content likely is).
%
In the following subsections, we will describe the intuition and novelty of each of our network's components.

==> sections/SpatialContextMod_v0.tex <==
\subsection{Spatial RGB Context Module}
\label{subsec:spat_rgb_ctxt_mod}

While inconsistent forensic residual is a sufficient indication of forgery in images, it is insufficient in videos~\cite{VideoFACT}. This is due to natural changes in compression strength induced by modern video codecs like H.264. These changes are influenced by a number of factors, including: local texture, lighting conditions, global coding parameters, etc.~\cite{VideoFACT, Jiang_2018_TIFS, Mandelli_2020_WIFS, Stamm_2010_ICIP} Hence, we need to capture spatial RGB context traces to condition the forensic residual evidence and increase the performance of our network.

We do this by passing the frame directly to a network $h_c$ that operates directly on the frame's RGB pixel values.
This network consists of a series of FIR blocks, followed by a final $1\times1$ convolutional layer to produce the final RGB Context Features: $C_t = h_c(\vframe_t)$.



==> sections/SpatialForensResidMod_v1.tex <==
\subsection{Spatial Forensic Residual Module}
\label{subsec:spat_forens_resid_mod}

This module is designed to extract evidence of manipulation from the spatial forensic residuals modality. Whenever content is inserted, edited, or synthesized, new noise-like microstructures are introduced and manifest themselves in this forensic modality. As a result, inconsistent forensic residuals is a well-adopted indication of forgery.

To best capture this trace, we create a rich set of learned forensic residuals using a constrained convolutional layer proposed in~\cite{MISLnet}. This layer is composed of a set of learnable prediction filters $\Phi^{f}$, whose output is subtracted from the pixel value being predicted.
%
These learned residuals are then analyzed using a subnetwork $h_f$ consisting of a series of fused inverted residuals (FIR) blocks~\cite{MobileNetV2} followed by a $1 \times 1$ layer,
%
to provide higher-level information for detecting spatial inconsistencies.  The resulting Spatial Forensic Residual Features are:
\skipless
\begin{equation}
	F_t= h_f(I_t\convolve(\delta-\Phi^f))
\end{equation}
where $\convolve$ denotes convolution and  $\delta$ is a unit impulse
(i.e. the convolutional identity element).
This architecture follows the ``squeeze-and-excitation'' network design principle in~\cite{SqueezeAndExcitation, EfficientNetV2}, which has been shown to capture rich, class-agnostic features in earlier layers, and specialize later layers towards high-level class-specific features.

To prevent this module from overfitting to scene content and maximize its generalizability over different manipulation types, we used a widely adopted approach of pretraining it to perform camera model identification using the Video-ACID dataset~\cite{Video-ACID}. However, unlike prior works which produce $F_t$ as a single embedding, our $F_t$ is a high dimensional dense feature set. Hence, to ensure the homogeneity of these features in frames from identical source, we introduce a novel adapter submodule and loss function. This submodule, $v$ contains multiple classifer heads, each corresponds to a pooling of features into embeddings at a different spatial resolution. The outputs of this submodule are likelihood scores from individual embeddings at all scales, $\theta_{i,j}^{k,c}$ for camera model $c$, where $i$ and $j$ denote the spatial index of the embedding at scale $k$. Finally, these multi-scale spatial decisions are aggregated to produce a novel pre-training loss function:
\begin{equation}
	\mathcal{L}_{\text{F}} = \sum_{k} \frac{-\lambda_k}{2^{2k}} \sum_{i,j} \sum_{c}
	\log\left(
	\frac{\exp(\theta^{k,c}_{i,j})\mathbbm{1}(c=c^*)}{\sum_{c} \exp(\theta^{k,c}_{i,j})} %\mathbbm{1}_{c=c^*}
	\right)
\end{equation}
where $c^*$ is the true source camera model, $\mathbbm{1}(\cdot)$ is the indicator function and $\lambda$ is the relative weight of each scale.
%In practice, we aggregate across three scales $k=\{3, 4, 5\}$ such that $\lambda_k= \{0.01, 0.0075, 0.005\}$.
After pretraining, we only retain $F_t$.





==> sections/SpatialMod_v0.tex <==
% SpatialMod_v0

\subsection{Spatial Forensic Feature Module}
\label{subsec:spatial_module}



When content within a scene is edited, synthesized, or falsified, new noise-like forensic microstructures are introduced~\cite{Noiseprint, MISLnet, FSG, FSM, VideoFACT}.  % Cite NoisePrint, lots of other stuff
As a result, the forensic microstructures in these regions are inconsistent with those distributed throughout the rest of the video frame.

Our spatial forensic module is designed to produce a set of features that can capture these spatially distributed microstructure inconsistencies within a single video frame.  To accomplish this, our spatial module consists of two parallel branches that produce distinct sets of features: learned forensic residual features and RGB context features.




\begin{comment}
Our network's spatial module generates two distinct intermediate feature sets: forensic residual features and RGB context features, derived from two parallel branches.

The first branch yields forensic residual features, instrumental in uncovering microstructures within video frames that indicate their processing history. In contrast, the second branch produces RGB context features, which complement the forensic residual features by providing local context. This integration is crucial as the distribution of forensic features is influenced by various factors like texture, lighting, compression, etc. Together, these feature sets offer a comprehensive and accurate forensic representation of a video frame.
\end{comment}

\subheader{Forensic Residual Features}
%
%This branch produces prediction residual features that reveal information about the video frame's origin and processing history.
Prediction residuals are an important forensic feature because they suppress a  frame's content while preserving noise-like microstructures introduced during by the camera %creation %(e.g., digital camera, AI generator)
and by subsequent editing.  %operations.
%
%

To best capture microstructures left by a variety of manipulations, we create a rich set of learned forensic residuals using a constrained convolutional layer proposed in~\cite{MISLnet}. This layer is composed of a set of learnable prediction filters $\Phi^{f}$, whose output is subtracted from the pixel value being predicted.
%
These learned residuals are then analyzed using a subnetwork $h_f$
consisting of a series of fused inverted residual (FIR) blocks~\cite{MobileNetV2} followed by a $1 \times 1$ layer, %$H_{f}$
to provide higher-level information for detecting spatial inconsistencies.  The resulting forensic residual features are
\pullup\pullup\pullup
\begin{equation}
%	\vspace{-0.5em}
    F_t= h_f(I_t\convolve(\delta-\Phi^f)),
    \pullup\pullup
\end{equation}
where $\convolve$ denotes convolution and  $\delta$ is a unit impulse (i.e. the convolutional identity element).
This architecture follows the ``squeeze-and-excitation'' network design principle in~\cite{SqueezeAndExcitation, EfficientNetV2}
% https://openaccess.thecvf.com/content_cvpr_2018/papers/Hu_Squeeze-and-Excitation_Networks_CVPR_2018_paper.pdf
%and \citethis
% http://proceedings.mlr.press/v139/tan21a.html
, which has been shown to
capture rich, class-agnostic features in earlier layers, and specialize later layers towards high-level class-specific features.
%The output of the last block is passed through a $1\times1$ convolutional layer to produce the final forensic residual features  $F_t$
% %, %$\Phi^f$ is the collection of learned prediction residual features,
%and $h_f(R)$ is the network used to learn the



\begin{comment}


%To best capture the microstructures left by a wide variety of manipulations, it is important to leverage a rich set of residuals specifically tuned for forensic purposes.
%Relying on a single or small set of fixed residual filters, as traditional networks often do, is unlikely to produce residuals that capable
%Our network accomplishes this by producing a set of learned forensic residuals using a constrained convolutional layer proposed by Bayar and Stamm~\citethis.  This layer comprises $L$ learnable prediction filters $\phi$, which produce a residual $\res^{(i)}$ for each filter:
\vspace{-0.5\baselineskip}
\begin{equation}
    \res^{(i)}=\vframe \convolve (\delta - \phi^{(i)}) %\; , \; i=1,2,\ldots,L
\end{equation}
where $\convolve$ denotes convolution and $\delta$ is a unit impulse, i.e. the convolutional identity element.

These learned residuals are then analyzed using a series of fused inverted residual (FIR) blocks \citethis , %$H_{f}$
to provide higher-level information for detecting spatial inconsistencies.
This architecture follows the ``squeeze-and-excitation'' network design principle in \citethis
% https://openaccess.thecvf.com/content_cvpr_2018/papers/Hu_Squeeze-and-Excitation_Networks_CVPR_2018_paper.pdf
and \citethis
% http://proceedings.mlr.press/v139/tan21a.html
, which has been shown to
capture rich, class-agnostic features in earlier layers, and specialize later layers towards high-level class-specific features.
The output of the last block is passed through a $1\times1$ convolutional layer to produce the final forensic residual features
%
\vspace{-0.5\baselineskip}
\begin{equation}
    %F = \textit{Conv1x1}(H_{f}(\res^{(i=1,2,\ldots,L)}))
    F_t= h_f(R),
\end{equation}
where $h_f(R)$ denotes the full network used to our forensic residual features.
%


\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%

To improve the performance of this branch, we pre-train it to perform forensic camera model identification using the Video-ACID dataset~\cite{Video-ACID}.
% before training the entire network.
As our ablation study shows, this pre-training step significantly improves the overall performance of our network. %, and enables it to learn higher quality forensic residual features.
 The pre-training procedure and loss is described in %further
 detail in %Sec.~\ref{subsec:ffe_pretrain}.
the supplemental material.



\subheader{RGB Context Features}
%
It is well known that the distribution and quality of forensic residual features can change based on a number of factors, including local texture, lighting conditions, compression strength, etc.~\cite{VideoFACT, Jiang_2018_TIFS, Mandelli_2020_WIFS, Stamm_2010_ICIP}.
%As a result, local information about the RGB content of a scene can provide important context to the network when making decisions based on these residual features.
%To exploit this information, our spatial module contains a second branch to capture local RGB context features to augment the forensic residual features learned by the first branch.  In this branch, the frame is passed directly to a network $h_c$ that operates directly on the frame's RGB pixel values.
To exploit this information, we capture local RGB context features to augment the forensic residual features by passing the frame directly to a network $h_c$ that operates directly on the frame's RGB pixel values.
This network consists of a series of FIR blocks, followed by a final $1\times1$ convolutional layer to produce the final context features $C= h_c(\vframe_t)$. %$C$ such that 	$C= h_c(\vframe_t)$.
\begin{comment}
\pullup\pullup
\begin{equation}
	C= h_c(\vframe).
	\pullup\pullup\pullup\pullup
\end{equation}
\end{comment}


\subheader{Combined  Spatial Forensic Features}
%
%Our spatial forensic feature module produces a final set of output features $S$ by concatenating the learned forensic residual and RGB context features such that
%
A final set of spatial forensic features $s$ are produced by concatenating the forensic residual and RGB context features so that $S = F \concat C$, where $\concat$ denotes the concatenation operator.
\begin{comment}
\pullup\pullup
\begin{equation}
    S = F \concat C.
    \pullup\pullup
\end{equation}
where $\concat$ denotes the concatenation operator.
\end{comment}

==> sections/TemporalForensResidMod_v1.tex <==
\subsection{Temporal Forensic Residual Module}
\label{subsec:temp_forens_resid_mod}

Many forms of video manipulation, especially AI-guided ones, change the content of each video frame individually. These algorithms often have a lesser emphasis on ensuring temporal consistency throughout the video. Because of this, the forensic microstructure at the location of the manipulated region can appear inconsistent when examined in a temporal manner.
While existing approaches have used some form of temporal information to identify these type of forgeries, none have tried to model the evolution, or change in forensic microstructures at a similar location over time.

To address this problem, we propose the Temporal Forensic Residual, a new forensic modality that is able to capture more general evidence of temporal inconsistencies in forensic microstructures. We do this by looking at how much do these microstructures change at each region across multiple adjacent frames. This is equivalent to computing the first order derivative, or, temporal residual, of the forensic feature field with respect to time. In particular,
%
our module calculates the difference of the current frame's forensic features compared to its previous frame, $\overrightarrow{T_t}$, and its subsequent frame, $\overleftarrow{T_t}$:
\begin{equation}
	\overrightarrow{T_t} = g_r(I_t) - g_r(I_{t-1}), \;\;
	\overleftarrow{T_t} = g_r(I_t) - g_r(I_{t+1})
\end{equation}
where $g_r$ is a lightweight CNN used to obtain the forensic feature field for each frame.
Then, we obtain the Temporal Forensic Residual features, $T_t$, by concatenating the forward and backward set of residual features, $\overrightarrow{T_t}$ and $\overleftarrow{T_t}$:
\begin{equation}
	T_t = \overrightarrow{T_t} \concat \overleftarrow{T_t}
\end{equation}
where $\concat$ represents the concatenation operation over the feature dimension.









%Existing approaches have tried to identify this inconsistency by directly modeling the sequence of forensic features. However, as we show in our experiments, these algorithms perform suboptimally when applied to a more general setting because it is impractical to learn all possible variations of abnormal and normal feature sequences.










==> sections/TemporalMod_v0.tex <==
% TemporalMod_v3_MCS
%
\subsection{Temporal Forensic Feature Module}
\label{subsec:TFFM}
%
Some video manipulations leave behind distinct forms of evidence that can be uncovered through temporal analysis.  These can correspond to small anomalous motions, inter-frame inconsistencies between forensic microstructures occurring at a common spatial location, minute small fluctuations in pixel intensity, etc.  This is especially possible if fake content in each frame is synthesized independently from other frames, as is done by several inpainting and deepfake techniques.


%these can correspond to minute anomalous motions, inter-frame inconsistencies between forensic microstructures occurring at a common spatial location, very small fluctuations in pixel intensity, etc. This is especially possible if fake content in each frame is synthesized independently from other frames, as is done by several inpainting and deepfake techniques~\citethis.


To capture these inconsistencies, the temporal module of our network contains two parallel branches that extract different sets of features: optical flow anomaly features and temporal residual inconsistency features.  These are then jointly analyzed to produce a set of temporal forensic features.  An overview of this branch can be seen in Fig.~\ref{fig:multi_res_pooling_arch}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%While falsified content may introduce spatially inconsistent forensic features,

%Some video manipulations may leave behind traces that can only be uncovered through temporal analysis

%For example, certain manipulations might introduce minute motion anomalies into a falsified region.

%Similarly, manipulations may leave behind forensic microstructures that are

%In an authentic video, forensic microstructures in a particular spatial location should be consistent across time.  By contrast, falsified video content may introduce inconsistencies in forensic microstructures that can be revealed by comparing them to microstructures in other frames at the same spatial location.  This is especially possible if fake content in each frame is synthesized independently from other frames, as is done by several inpainting and deepfake techniques~\citethis.



%This is especially possible if fake content in each frame is synthesized independently from other frames, as is done by some inpainting and deepfake techniques~\citethis.

%To capture these inconsistencies, the temporal module of our network contains two parallel branches that extract different sets of features: optical flow anomaly features and temporal residual inconsistency features.  These are then jointly analyzed to produce a set of temporal forensic features.



\subheader{Optical Flow Anomaly Features}
%
%Some video manipulations introduce minute anomalous motions into a falsified video.  This is especially possible if fake content in each frame is synthesized independently from other frames, as is done by some inpainting and deepfake techniques~\citethis.
%
%To capture these anomalous motions, we extract a set of optical flow anomaly features.
We extract a set of optical flow features to capture anomalous motions.
%
%
%Specifically, we obtain the forward optical flow $O_{t}^{\rightarrow}$ from the previous frame $I_{t-1}$  and the backward optical flow $O_{t}^{\leftarrow}$ from the subsequent frame $I_{t+1}$ according to
Specifically, we obtain the forward optical flow from the previous frame $O_{t}^{\rightarrow}$ and the backward optical flow from the subsequent frame $O_{t}^{\leftarrow}$ according to
\begin{equation}
 O_{t}^{\rightarrow} = \nu(I_{t}, I_{t-1}), \;\;
        O_{t}^{\leftarrow} = \nu(I_{t}, I_{t+1}),
\end{equation}
where $\nu(X,Y)$ computes the optical flow from $Y$ to $X$.  In practice, we compute these optical flows using RAFT~\cite{RAFT}.

\subheader{Temporal Residual Inconsistency Features}
%
%To capture inconsistencies in forensic microstructures across time,
To capture other temporal inconsistencies,
such as changes in forensic microstructures across time as well as pixel intensity flickering,
we first extract a set of temporal residual features.  This is done by producing learned residuals using a constrained convolutional layer, then obtaining higher-level residual features using a convolutional network $g_r$.  As a result, the temporal residual features at frame $I_t$ are
\begin{equation}
P_t= g_r(I_t*(\delta-\Phi)),
\end{equation}
where $\Phi$ is the collection of learned prediction filters in this network's constrained convolutional layer. We utilize a different network than the one used to produce spatial forensic residual features because temporal variations in microstructures may take a different form than spatial variations.
Next, we obtain the forward $W_{t}^{\rightarrow}$ and backward $W_{t}^{\leftarrow}$ temporal inconstancy in these residual features  according to
\begin{equation}
W_{t}^{\rightarrow} = P_{t} - P_{t-1}, \;\;
        W_{t}^{\leftarrow} = P_{t} - P_{t+1}. \\
\end{equation}

\subheader{Temporal Forensic Features}
After obtaining the set of optical flow anomaly features and temporal residual inconsistency features, we join them together and learn higher-level temporal forensic features.  This is done by passing the concatenated features through a network $g_\tau$ consisting of a single convolutional layer
such that
\begin{equation}
T_{t}= g_\tau(O_{t}^{\rightarrow}  \concat O_{t}^{\leftarrow} \concat W^{\rightarrow} \concat W_{t}^{\leftarrow}).
\end{equation}





==> sections/TemporalOptFlowResidMod_v1.tex <==
\subsection{Optical Flow Residual Module}
\label{subsec:opt_flow_resid_mod}

Some forms of video manipulation, such as AI-guided inpainting, may leave behind anomalous motion patterns.
Specifically, when an object moves but not all optical flow vectors from that object are moving in the same direction.
This phenomenon occurs due to inaccuracies of existing algorithms in modeling object motion with possible occlusions.
%
Some prior works~\citethis have tried to directly use optical flow vectors to search for motion anomalies. These approaches often fall short because it is impractical to model all forms of authentic and anomalous optical flow in all videos under various scene conditions and rate of motions.

Therefore, using similar intuition as in Sec.~\ref{subsec:temp_forens_resid_mod}, we address this problem by first extracting the temporal residuals of the optical flow in both forward, $\overrightarrow{O_t}$, and backward, $\overleftarrow{O_t}$, directions:
\begin{equation}
	\overrightarrow{O_t} = \nu (I_t, I_{t-1}) - \nu (I_{t-1}, I_{t-2}), \;\;
	\overleftarrow{O_t} = \nu (I_t, I_{t+1}) - \nu (I_{t+1}, I_{t+2})
\end{equation}
where $\nu$ is the metwork RAFT~\cite{RAFT}, an optical flow extractor.
Then, to obtain the Optical Flow Residual features, we concatenate the forward and backward optical flow temporal residuals:
\begin{equation}
	O_t = \overrightarrow{O_t} \concat \overleftarrow{O_t}
\end{equation}









==> sections/Transformer_v0.tex <==
% Transformer_v3_MCS
%
\subsection{Transformer-Based Self-Attention Module}
\label{subsec:transformer}

In order to detect and localize fake content, it is necessary to identify forensic embeddings that are inconsistent with the rest.
To facilitate this, we utilize a transformer~\cite{OGTransformer} module consisting of eight stacked encoder blocks.

The input to the first %transformer
encoder block is the sequence of multi-scale spatio-temporal embeddings. Learned position embeddings~\cite{ViT} $E_{pos}$ are added to this sequence to produce a set of tokens $Z_{t}$, which are then passed through a multi-head self-attention layer (MHSA).  This produces  a sequence of contextualized tokens $Z'_{t}$ such that
%
\begin{align}
%        Z_{t}& = [ \xi_t(0,0);\xi_t(0,1); \cdots ; \xi_t(0,2^k); \cdots ; \xi_t(2^k,2^k) ] + E_{pos}, \\
%Z_{t}& = [ \xi_t(1);\ldots; \xi_t(N)] + E_{pos} \\
Z_{t}& = [ \xi_t(1,1);\ldots; \xi_t(M,N)] + E_{pos}, \\
        Z_{t}^{'}& = \text{MHSA}(Z_{t}) + Z_{t}.
\end{align}
%After this, the sequence of tokens are passed through an MLP layer to produce a set of new forensic features $Y^{(1)}_t$ that are contextualized through self-attention
After this, the sequence of tokens is passed through an MLP layer to produce a new set of higher-level contextualized forensic features $Y^{(1)}_t$  such that:
%that have been contextualized through self-attention
%
\begin{equation}
Y_{t}^{(1)} = \text{MLP}(Z_{t}^{'}) + Z_{t}^{'}
\end{equation}
These features are further passed through a series of stacked encoder blocks to produce a final set of high order contextualized forensic features $Y^{(L)}$.
%
This enables our module to capture complex relationships between lower-level embeddings and produce higher-level features that are able to expose subtle forensic inconsistencies.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\hrulefill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
Obtained from the preceding module is a sequence of multi-scale embedings that capture spatial and temporal traces for each analysis region
. The key to detecting and localizing fake content is identifying which embeddings display inconsistencies relative to others. Here, the Transformer architecture's Self-Attention mechanism excels, effectively putting all embeddings in context of each other to uncover inconsistencies.
%This method allows for precise identification of regions that are either consistent with real content or reveal falsification through their high-quality yet incongruent information.
%The Self-Attention process is formulated as:
This mechanism is encapsulated by:
% insert multi-headed transformer equation here
\begin{equation}
    \begin{split}
        Z_{t} = [ \xi_t^{0,0};\xi_t^{0,1}; \cdots ; \xi_t^{0,2^k}; \cdots ; \xi_t^{2^k,2^k} ] + E_{pos} \\
        Z_{t}^{'} = \text{MHSA}(Z_{t}) + Z_{t}
    \end{split}
\end{equation}
with $E_{pos}$ being the learnable positional embeddings.
%
Further transformation of these embeddings is performed by the MLP layers within the Transformer block, enhancing them to a higher-level representation:
% insert MLP equation here
\begin{equation}
    \begin{split}
        Y_{t}^{0} = \text{MLP}(Z_{t}^{'}) + Z_{t}^{'}
    \end{split}
\end{equation}
These higher-level embeddings are then refined through a series of $N$ Transformer blocks, denoted as $B$. The culmination of this is a set of advanced, contextually enriched forensic embeddings, optimized for the task of detecting and localizing fake content:
\begin{equation}
    \begin{split}
        Y_{t}^{N} = B^{N-1} \circ \cdots \circ B^{0}(Z_{t})
    \end{split}
\end{equation}
where $\circ$ denotes the function composition operation.
\end{comment}

==> tables/dataset_statistics.tex <==

\begin{table*}[!tbh]
	\caption{\label{table:dataset_statistics} Dataset statistics of the \pooleddsname Dataset.}
    \centering
    \resizebox{1.0\linewidth}{!}{%
        \begin{tblr}{
            width = \linewidth,
            colspec = {|t{45mm}|t{15mm}|t{29mm}|t{29mm}|t{29mm}|t{13mm}|t{18mm}|},
            column{2} = {l},
            column{3} = {r},
            column{4} = {r},
            column{5} = {r},
            vline{2-3,6} = {-}{},
            hline{1,2,7,8} = {-}{},
        }
            \textbf{ Dataset Source }
            & \textbf{ Manip. Type }
            & \textbf{ Training Frames (Videos) per CRF }
            & \textbf{ Validation Frames (Videos) per CRF }
            & \textbf{ Testing Frames (Videos) per CRF }
            & \textbf{Training CRF}
            & \textbf{Testing CRF} \\
            VideoFACT Std. Manips.~\cite{VideoFACT}         & Splicing
            & 180,000 (6,000) & 18,000 (600) & 36,000 (1,200) & 0, 23 & 0, 10, 23, 28 \\
            VideoFACT Std. Manips.~\cite{VideoFACT}         & Editing
            & 180,000 (6,000) & 18,000 (600) & 36,000 (1,200) & 0, 23 & 0, 10, 23, 28 \\
            FaceForensics++~\cite{FF++}   & Deepfake
            & 90,000 (1,538) & 9,000 (154) & 18,000 (308) & 0, 23 & 0, 10, 23, 28 \\
            DeepFakeDetection~\cite{DFD}  & Deepfake
            & 90,000 (552) & 9,000 (52) & 18,000 (112) & 0, 23 & 0, 10, 23, 28 \\
            DEVIL Dataset~\cite{DEVIL}            & Inpainting
            & 100,922 (1,150) & 9,620 (110) & 20,802 (240) & 0, 23 & 0, 10, 23, 28 \\
            \textbf{Total per CRF}    & \textbf{Various}
            & \textbf{640,922 (15,240)} & \textbf{63,620 (1,561)} & \textbf{128,802 (3060)} & 0, 23 & 0, 10, 23, 28
        \end{tblr}
    }

\end{table*}

==> tables/training_hyperparameters.tex <==

\begin{table}[!t]
    \centering
    \caption{\label{table:training_hyperparameters} Training hyperparameters of our approach.}
    \resizebox{\linewidth}{!}{%
        \begin{tblr}{
            width = \linewidth,
            colspec = {|t{7mm}|t{16mm}|t{30mm}|t{13mm}|t{15mm}|t{12mm}|t{18mm}|},
            cell{2-4}{1} = {c},
            cell{2}{4-7} = {c},
            cell{3}{4-7} = {c},
            cell{4}{4-7} = {c},
            vline{1-4,8} = {-}{},
            hline{1-2,5} = {-}{},
        }
        Stage & Frozen Module & Training Module & Optimizer & Initial LR & Moment. & Step decay\\
        1 & N/A & FFE & SGD & 1.00E-03 & 0.96 & 0.65 every 2\\
        2 & FFE & All but FFE \& TIM & SGD & 8.00E-04 & 0.90 & 0.65 every 2\\
        3 & RAFT & All & SGD & 2.00E-04 & 0.90 & 0.75 every 2
        \end{tblr}
    }
\end{table}
